Risk Verification of Stochastic Systems with Neural Network Controllers

Motivated by the fragility of neural network (NN) controllers in safety-critical applications, we present a data-driven framework for verifying the risk of stochastic dynamical systems with NN controllers. Given a stochastic control system, an NN controller, and a specification equipped with a notion of trace robustness (e.g., constraint functions or signal temporal logic), we collect trajectories from the system that may or may not satisfy the specification. In particular, each of the trajectories produces a robustness value that indicates how well (severely) the specification is satisfied (violated). We then compute risk metrics over these robustness values to estimate the risk that the NN controller will not satisfy the specification. We are further interested in quantifying the difference in risk between two systems, and we show how the risk estimated from a nominal system can provide an upper bound the risk of a perturbed version of the system. In particular, the tightness of this bound depends on the closeness of the systems in terms of the closeness of their system trajectories. For Lipschitz continuous and incrementally input-to-state stable systems, we show how to exactly quantify system closeness with varying degrees of conservatism, while we estimate system closeness for more general systems from data in our experiments. We demonstrate our risk verification approach on two case studies, an underwater vehicle and an F1/10 autonomous car.

==> chapter/background.tex <==
\section{Background and Problem Formulation OLD}
\label{sec:backgound_old}

True and false are encoded as $\top:=\infty$ and $\bot:=-\infty$, respectively, with the set $\mathbb{B}:=\{\top,\bot\}$. Let $\mathbb{R}$ and $\mathbb{N}$ be the set of real and natural numbers, respectively, with $\mathbb{N}$ including zero. Also let $\mathbb{R}_{\ge 0}$ be the set of non-negative real numbers and $\mathbb{R}^n$ be the real $n$-dimensional vector space.    For  $a,b\in\mathbb{R}$, let
\begin{align*}
\mathbb{I}(a\le b):=\begin{cases}
1 &\text{if } a\le b\\
0 &\text{otherwise}
\end{cases}
\end{align*} 
be the indicator function indicating whether or not $a\le b$. Let $\mathfrak{F}(T,S)$ denote the set of all measurable functions mapping from the domain $T$ into the domain $S$, i.e., $f\in \mathfrak{F}(T,S)$ is a measurable function $f:T\to S$.   
%\textcolor{red}{Define class K and KL functions for definition of iISS.f}

We also introduce the definitions of class $\mathcal{K}$, $\mathcal{K}_{\infty}$, $\mathcal{L}$, and $\mathcal{K}\mathcal{L}$ functions, which are used in defining and analyzing incremental input to state stable systems.

\begin{definition} \label{def:classK}
A function $\alpha : \mathbb{R}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ is said to be of class-$\mathcal{K}$ ($\alpha \in \mathcal{K}$) if it is continuous, strictly increasing and $\alpha(0)=0$.  
\end{definition}

\begin{definition} \label{def:classKInfty}
A function $\alpha : \mathbb{R}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ is said to be of class-$\mathcal{K}_{\infty}$ ($\alpha \in \mathcal{K}_{\infty}$) if $\alpha \in \mathcal{K}$ and $\text{lim}_{s\rightarrow \infty} \; \alpha(s)=\infty$.
\end{definition}


\begin{definition}
A function $\sigma : \mathbb{R}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ is said to be of class-$\mathcal{L}$ ($\sigma \in \mathcal{L}$) if it is continuous, strictly decreasing, and $\text{lim}_{s \rightarrow \infty} \; \sigma(s) = 0$.
\end{definition}

\begin{definition}\label{def:classKL}
A function $\beta : \mathbb{R}_{\geq 0} \times \mathbb{R}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ is said to be of class $\mathcal{K}\mathcal{L}$ ($\beta \in \mathcal{K}\mathcal{L}$) if it is class-$\mathcal{K}$ in its first argument and class-$\mathcal{L}$ in its second argument.
\end{definition}


\subsection{Random Variables, Risk Measures, and Stochastic Processes}
\label{sec:stoch}
Consider the \emph{probability space} $(\Omega,\mathcal{F},P)$  where $\Omega$ is the sample space, $\mathcal{F}$ is a $\sigma$-algebra of $\Omega$, and $P:\mathcal{F}\to[0,1]$ is a probability measure. More intuitively, an element in  $\Omega$ is an \emph{outcome} of an experiment, while an element in $\mathcal{F}$ is an \emph{event} that consists of one or more outcomes whose probabilities can be measured by the probability measure $P$. 

 Let $Z$ denote a real-valued \emph{random vector}, i.e., a measurable function $Z:\Omega\to\mathbb{R}^n$. A \emph{risk measure} is a function $R:\mathfrak{F}(\Omega,\mathbb{R})\to \mathbb{R}$ that maps from the set of real-valued random variables to the real numbers. The value of $R(Z)$  quantifies the risk associated with a cost random variable $Z:\Omega\to\mathbb{R}^n$.  Risk measures hence allow for a risk assessment in terms of such cost random variables. Commonly used risk measures are the expected value, the variance, the value-at-risk, or the conditional value-at-risk \cite{rockafellar2000optimization}. A particular property of $R$ that we need in this paper is \emph{monotonicity} and \emph{translational invariance}:
 \begin{itemize}
     \item For two cost random variables $Z,Z'\in \mathfrak{F}(\Omega,\mathbb{R})$, the risk measure $R$ is monotone if $Z(\omega) \leq Z'(\omega)$ for all $\omega\in\Omega$ implies that $R(Z) \le R(Z')$.
     \item For a random variables $Z\in \mathfrak{F}(\Omega,\mathbb{R})$, the risk measure $R$ is translationally invariant if, for a constant $c\in\mathbb{R}$, it holds that $R(Z + c) = R(Z) + c$.
 \end{itemize} 
\begin{remark}
In \ref{app:risk}, we summarize other desireable properties of $R$ such as positive homogeneity, subadditivity, commotone additivity, and law invariance. We also provide a summary of existing risk measures and emphasize that our presented method is compatible with any of these risk measures as long as they are  monotone and translationally invariant.
\end{remark} 

For a time domain $\mathbb{T}\subseteq \mathbb{N}$, a \emph{stochastic process} is a function $X:\mathbb{T}\times \Omega \to \mathbb{R}^n$ where  $X(t,\cdot)$ is a random vector for each fixed $t\in \mathbb{T}$. A stochastic process can   be viewed as a collection of random vectors $\{X(t,\cdot)|t\in \mathbb{T}\}$  that are defined on a common probability space $(\Omega,\mathcal{F},P)$.  For a fixed $\omega\in\Omega$, the function $X(\cdot,\omega)$ is a \emph{realization} of the stochastic process. We already remark that stochastic dynamics systems, as defined in the next section, are a particular form of a stochastic process.
 
 %We refer to $X$ as continuous-space stochastic process when the CDF of $X(t,\cdot)$ is continuous and as discrete-space stochastic process otherwise.  













==> chapter/case_studies_risk_gap.tex <==
\section{Case Studies}
\label{sec:simulations}

We continue our empirical validation of the F1/10 car and the (UUV) by running experiments to quantify the risk gap for these two systems.



\subsection{F1/10 Car}

This subsection continues the F1/10 case study introduced in Section~\ref{sec:F1TenthCaseStudy1}. In that portion of the case study, we used the statistical risk verification framework introduced in Section~\ref{risskk} to test 6 different NN controllers on a simulated model of the system. Now we analyze the same NN controllers on a more realistic LiDAR model and compare the results to the theory from Section~\ref{sec:risk_gap}.

%The second case study concerns an F1/10 car driving through a hallway with occasional turns. The car is equipped with a LiDAR system for sensing the distances to the hallway.  The STL requirement is specified with the following STL formula:
%\begin{align} \label{eq:F10spec_2}
%\phi_{F1/10} := G \left(d>d_{w} \right)
%\end{align}
%where $d$ is the distance of the car to the nearest wall and $d_w$ is the minimum allowed distance from the car to the wall.

%We trained 6 different NN controllers for navigating the car through the hallway, taking LiDAR rays as input and giving steering commands as output. We used a standard bicycle model as the model of the car for performing the RL. Our LiDAR model consisted of noisy range values and a fixed probability of a LiDAR randomly getting dropped before each trial.\footnote{A common issue with using LiDAR is that the rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We refer to this as a 'dropped' ray.} The specification for the car is that it never collides with the walls of the hallway, which is given in equation \eqref{eq:F10spec_2}. %We then ran 50000 trials of each controller navigating through a hallway with a right hand turn. 

%A common issue with using LiDAR data is that each LiDAR ray can be quite noisy. For example, the LiDAR rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We accounted for this behavior in two ways. First, we altered our LiDAR model to randomly choose rays to drop for the duration of each run and ran 50000 trials for each controller. %From these data, we computed the VaR and CVaR risks for each of the controllers, which are shown in figure \ref{ex:f1-10VarMissingRays} and figure \ref{ex:f1-10CVarMissingRays}, respectively.

To simulate real-world LiDAR data, we  trained a GAN to approximate LiDAR readings from real-world LiDAR data. The GAN had a deconvoluational NN architecture \cite{radford2016} and was trained using the Wasserstein GAN algorithm \cite{arjovsky2017,gulrajani2017}. The GAN takes in the position and heading of the car and a 10 dimensional (random) seed and outputs an array of 21 LiDAR rays. 

Equation \eqref{eq:f1tenthsystemganlidar} shows the F1-10th with GAN LiDAR. The dynamics $f$ and state $\overline{X}$ are the same as in Section~\ref{sec:F1TenthCaseStudy1}. The GANLiDAR function is the GAN LiDAR model.
\begin{subequations}\label{eq:f1tenthsystemganlidar}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{DNN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{GANLiDAR}(\overline{X}(t)),
\end{align}
\end{subequations}

We now rewrite equation \eqref{eq:f1tenthsystemganlidar} to match the form of \eqref{eq:system_real}. The $W$ term accounts for the measurement differences between the simulated LiDAR and the GAN LiDAR. There is no $V$ term here, since the dynamics of the two system models are equivalent. 
\begin{subequations}\label{eq:f1tenthsystemganlidarerr}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{DNN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{SiMLiDAR}(\overline{X}(t)) + W(\overline{X}(t),\cdot),
\end{align}
\end{subequations}
where $W(\overline{X}(t),\cdot)=\text{GaNLiDAR}(\overline{X}(t)) - \text{SiMLiDAR}(X(t))$.






With this equation in hand, we ran 50000 trials of each of the 6 NN controllers operating in a hallway. From these data, we computed the VaR and CVaR risks for each of the controllers and LiDAR models using a single risk level of $\beta:=0.9$ and confidence of $1-\delta:=0.95$, which are shown in tables \ref{Tab:f1tenthVars} and \ref{Tab:f1tenthCVars}, along with the VaR and CVaR values from \eqref{eq:f1tenthsystemsimlidar} for ease of comparison.



\begin{table*}[h]
\caption{F1/10 VaR values for different LiDAR models under the specification given in \ref{eq:F10spec}.}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline Controller Name & Controller Type & Simulated LiDAR  & GAN Lidar & Color in Figures  \\ \hline
    1 & DDPG 64x64 & 0.1050 & 0.1306 & Black \\ \hline
    2 & TD3 64x64 & 0.0776 & 0.0944 & Red \\ \hline
    3 & DDPG 128x128 & 0.1483 & 0.1435 & Green \\ \hline
    4 & DDPG 64x64 & 0.0165 & 0.1140 & Blue\\ \hline
    5 & TD3 128x128 & 0.0368 & 0.0801 & Magenta\\ \hline
    6 & TD3 64x64 & 0.0300 & 0.0727 & Cyan \\
    \hline
    \end{tabular}
    \label{Tab:f1tenthVars}
\end{table*}



\begin{table*}[h]
\caption{F1/10 CVaR values for different LiDAR models under the specification given in \ref{eq:F10spec}.}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline Controller Name & Controller Type & Simulated LiDAR  & GAN LiDAR & Color in Figures  \\ \hline
    1 & DDPG 64x64 & 0.1392 & 0.1986 & Black \\ \hline
    2 & TD3 64x64 & 0.1108 & 0.1321 & Red \\ \hline
    3 & DDPG 128x128 & 0.1892 & 0.2038 & Green \\ \hline
    4 & DDPG 64x64 & 0.0805 & 0.1689 & Blue \\ \hline
    5 & TD3 128x128 & 0.0746 & 0.1286 & Magenta \\ \hline
    6 & TD3 64x64 & 0.0640 & 0.1249 & Cyan \\
    \hline
    \end{tabular}
    \label{Tab:f1tenthCVars}
\end{table*}


% simulation vars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_dont_hit_wall.png}
%\caption{Value-at-Risks (VaRs) for the STL robustness of 12 different RL-training f1tenth controllers.}
%\label{fig:f1-10Var}
%\end{figure}

% simulation cvars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_dont_hit_wall.png}
%\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness of 12 different RL-training f1tenth controllers.}
%\label{fig:f1-10CVar}
%\end{figure}

% missing lidar rays vars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_dont_hit_wall_missingRays.png}
%\caption{Value-at-Risks (VaRs) for the STL robustness of 12 different RL-training f1tenth controllers while randomly dropping lidar rays.}
%\label{fig:f1-10VarMissingRays}
%\end{figure}

% missing lidar rays cvars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_dont_hit_wall_missingRays.png}
%\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness of 12 different RL-training f1tenth controllers while randomly dropping lidar rays.}
%\label{fig:f1-10CVarMissingRays}
%\end{figure}


% gan vars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_dont_hit_wall_gan.png}
%\caption{Value-at-Risks (VaRs) for the STL robustness of 12 different RL-training f1tenth controllers, using a GAN to generate artificial LiDAR data.}
%\label{fig:f1-10VarGan}
%\end{figure}

% gan cvars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_dont_hit_wall_gan.png}
%\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness of 12 different RL-training f1tenth controllers, using a GAN to generate artificial LiDAR data.}
%\label{fig:f1-10CVarGan}
%\end{figure}



%In addition, we ran several real world traces (between 8 and 10) of the 12 controllers, for both modified and unmodified environments. The crash chances for each controller are shown in figures below.

%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/uncoveredCrashChances.png}
%\caption{Crash chances of the controllers for a clean environment.}
%\label{fig:f1-10Var}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/coveredCrashChances.png}
%\caption{Crash chances of the controllers for a modified environment.}
%\label{fig:f1-10CVar}
%\end{figure}

%All of the various var and cvars values are shown in the tables below.



We see that the controllers which perform well on the LiDAR model also perform well on the GAN LiDAR model, which is expected.





%With these two equations (\eqref{eq:f1tenthsystemsimlidar} and \eqref{eq:f1tenthsystemganlidarerr}) in hand, we generated 50000 traces for each of the 6 NNs we trained to guide the F1/10 car through a hallway with a right-hand turn.

%Second, we trained a GAN to approximate more realistic LiDAR readings using data of a real F1/10 car travelling around hallways. The GAN takes in the position and heading of the car and a 10 dimensional (random) seed and outputs an array of 21 LiDAR rays. Using this GAN, we then ran 50000 trials of each of the 12 NN controllers operating in a hallway. %From these data, we computed the VaR and CVaR risks for each of the controllers, which are shown in figure \ref{ex:f1-10VarGan} and figure \ref{ex:f1-10CVarGan}, respectively.  




%The GAN based lidar var values are consistent with the real world crash chances, which demonstrates how the risk robustness helps in addressing the sim2real gap.



Next, we varied the $\beta$ values for the VaR and CVaR metrics. These $\beta$ values control how much or little of the tail gets considered in the risk. Larger values only consider the extremes of the tails. The figures below show the different risk values for various controllers for both the simulated and GAN lidar models. Each controller gets its own color and the simulated LiDAR model values are shown as dots and the GAN LiDAR values are shown as stars. Note that we still observe that the controllers which perform better on the simulated LiDAR also perform well on the GAN LiDAR, although the correlation is not as clean as with the UUV case study. In particular, the blue controller shows very good CVaR values for smaller $\beta$ values, but as $\beta$ increases the performances becomes dominated by other controllers. The blue controller then performs much worse than those controllers on the GAN data. This illustrates the benefit of using risk measures analyzing systems in simulation. The very poor performance of the blue controller at the extreme tails of its robustness distribution properly indicated that it would not generalize well to the GAN LiDAR model.

\begin{figure}
\centering
\includegraphics[scale=0.5]{document/figures/vars_simReal_diffBetas.png}
\caption{Value at Risks (VaRs) for the F1/10 car under the specification given in \ref{eq:F10spec} for the simulated and GAN lidar models and various controllers.}
\label{fig:f1-10VarManyBetas}
\end{figure}


\begin{figure}
\centering
\includegraphics[scale=0.5]{document/figures/cvars_simReal_diffBetas.png}
\caption{Conditional Value at Risks (CVaRs) for the F1/10 car under the specification given in \ref{eq:F10spec} for the simulated and GAN lidar models and various controllers.}
\label{fig:f1-10CVarManyBetas}
\end{figure}



%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_simlidar_diffBetas.png}
%\caption{Value at Risks (VaRs) for the f1tenth car under specification 'do not hit the wall' for the simulated lidar model and various controllers.}
%\label{ex:f1-10SimLidarVarManyBetas}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_simlidar_diffBetas.png}
%\caption{Conditional Value at Risks (CVaRs) for the f1tenth car under specification 'do not hit the wall' for the simulated lidar model and various controllers.}
%\label{ex:f1-10SimLidarCVarManyBetas}
%\end{figure}



%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_missingrays_diffBetas.png}
%\caption{Value at Risks (VaRs) for the f1tenth car under specification 'do not hit the wall' for the 'missing rays' lidar model and various controllers.}
%\label{ex:f1-10MissingRaysVarManyBetas}
%\end{figure}



%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_missingrays_diffBetas.png}
%\caption{Conditional Value at Risks (CVaRs) for the f1tenth car under specification 'do not hit the wall' for the 'missing rays' lidar model and various controllers.}
%\label{ex:f1-10MissingRaysCVarManyBetas}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_gan_diffBetas.png}
%\caption{Value at Risks (VaRs) for the f1tenth car under specification 'do not hit the wall' for the GAN lidar model and various controllers.}
%\label{ex:f1-10GANVarManyBetas}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_gan_diffBetas.png}
%\caption{Conditional Value at Risks (VaRs) for the f1tenth car under specification 'do not hit the wall' for the GAN lidar model and various controllers.}
%\label{ex:f1-10GANCVarManyBetas}
%\end{figure}






\subsection{Unmanned Underwater Vehicle (UUV)}


This subsection continues the UUV case study introduced in Section \ref{sec:UUVlin}.



%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.25]{document/figures/uuv/uuv_figure_topdown.png}
%\caption{The UUV operating environment, both on paper and in the high fidelity physics engine. The pipelines are both shown in blue.}
%\label{fig:uuv_fig}
%\end{figure}


%The UUV is tasked with following alongside a pipeline on the seafloor and using a side-scan sonar system to capture and inspect the pipeline, as shown in Figure \ref{fig:uuv_fig}. As the sonar works best in a certain range of distances from the pipeline, we consider the following requirement in STL that expresses expeditiousness:
%\begin{align} \label{eq:UUVspec}
%    \Phi_{UUV}:= &G (d<d_{u} \lor F_{[0,t_{UUV}]} d<d_{u}) \land \\
%    &G (d>d_{l} \lor F_{[0,t_{UUV}]} d>d_{l}) \nonumber
%\end{align}
%\begin{align} \label{eq:UUVspec}
%    \Phi_{UUV}:= &G \left[d<d_l \implies F_{[0,t_{UUV}]} \left(d \geq d_l \right) \right] \land \\
%    &G \left[d>d_u \implies F_{[0,t_{UUV}]} \left(d \leq d_u \right) \right] \nonumber
%\end{align}
%\textcolor{red}{1) Use STL terminology from background section, $F$ instead of $\square$, 2) use implication operator instead of disjunction re-formulation for better understanding - only few people are aware of the re-formulation.}
%where $d$ is the UUV's distance to the pipeline in the plane, $d_u$ and $d_l$ are the upper and lower distances to the pipe which the UUV must lie within and $t_{UUV}$ is the amount of time in which the UUV is allowed to leave this distance range.\footnote{For example, the UUV may need to avoid obstacles, in which case it is allowed to lose the pipe for a small period of time.}



%We consider a high-fidelity UUV model based on the ROS-Gazebo real-time physics engine presented in \cite{Manhaes2016}. As gathering data on real-time systems is time-consuming, we view this model as the perturbed system in \eqref{eq:system_real} and we will instead derive a linearized model corresponding to \eqref{eq:system} next that we can use to collect data more efficiently. In the end, however, we will collect data from both systems to support the claims made in Section \ref{sec:risk_gap} with respect to the risk gap between the systems in \eqref{eq:system} and \eqref{eq:system_real}.

We consider a high-fidelity UUV model based on the ROS-Gazebo real-time physics engine presented in \cite{Manhaes2016} as the perturbed system in \eqref{eq:system_real}\footnote{Recall that we used a linearization of the real time physics engine as our nominal system.}.

 
The equations in \eqref{eq:uuvsystemphys} show the real-time physics engine UUV dynamics. In this case, $Y(t) = \begin{bmatrix} d \\ \theta \end{bmatrix}$ is the distance and heading of the UUV with respect to the pipeline being tracked. The dynamics $f$ and state $X(t)$ are internal to the real-time physics engine, so we keep them general due to space constraints. The SSS function stands for side scan sonar, which is what the UUV uses to detect and track the pipeline. Finally, the DNN function is our DNN controller for the UUV.
\begin{subequations}\label{eq:uuvsystemphys}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{DNN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{SSS}(\overline{X}(t)),
\end{align}
\end{subequations}

For clarity, we restate the dynamics of the linear UUV simulator below.
%The equations in \eqref{eq:uuvsystemlin} show the dynamics of the linear simulator of the UUV. Here we have replaced the original dynamics $f$ with the linearized dynamics $f_{lin}$. The linearization also reduces the number of internal UUV states; so we have $\overline{X} = \begin{bmatrix} x_{uuv} & y_{uuv} & \theta_{uuv} &  v_{uuv} & d_{uuv} \end{bmatrix} ^{T}$, which contains the 2-D position, heading, speed and depth of the UUV, respectively. The $V$ term represents the linearization error of the system. Note that there is no measurement error term $W$, since the linearization does not affect the UUV sonar.
 \begin{subequations}\label{eq:uuvsystemlin_2}
\begin{align}
    X(t+1)&=f_{lin}(C(t),\text{DNN}(Y(t))), \; X(0)=X_0\\
    Y(t)&=\text{SSS}(X(t))
\end{align}
\end{subequations}


In order to get equations \eqref{eq:uuvsystemphys} and \eqref{eq:uuvsystemlin_2} to resemble equations \eqref{eq:system} and \eqref{eq:system_real}, we rewrite \eqref{eq:uuvsystemphys} as
\begin{subequations}\label{eq:uuvsystemphyserr}
\begin{align}
    \overline{X}(t+1)&=f_{lin}(\overline{X}(t),\text{DNN}(\overline{Y}(t)))+V(\overline{X}(t),\cdot),  \; \overline{X}(0)=X_0,\\
    \overline{Y}(t)&=\text{SSS}(\overline{X}(t)),
\end{align}
\end{subequations}

So we have replaced the real-time physics engine as the linear simulator plus some linearization error term $V(\overline{X}(t),\cdot)$.

%Having systems \eqref{eq:uuvsystemlin_2} and \eqref{eq:uuvsystemphyserr} at hand, our ultimate goal is to verify DNN controllers that have been trained for these systems and with the objective in \eqref{eq:UUVspec}. In particular, we  used the Twin Delayed Deep Deterministic Policy Gradients (TD3) algorithm \cite{Fujimoto2018} to train 4 NN controllers for guiding the UUV alongside a pipeline on the seafloor. The reward function for the RL used 4 additive terms. The first term gave a small penalty for each simulation step. The next gave a penalty for the magnitude of the commanded change in heading from the controller. The third gave a penalty for the difference between the UUV's distance to the pipeline and the desired distance to the pipeline. The final term adds a very large penalty if the UUV's distance to the pipe gets outside some safe interval. The size of the safe interval is what we altered for training the controllers. 

Having systems \eqref{eq:uuvsystemlin_2} and \eqref{eq:uuvsystemphyserr} at hand, our ultimate goal is to experimentally compute the risk gaps for each of the 4 DNN controllers we trained in section \ref{sec:UUVlin}. To do this, we collected 300 runs of the real-time physics engine, each corresponding to 3 minutes of data per run. Finally, the STL robustness risk of the STL specification in \eqref{eq:UUVspec} is estimated as explained in Section ~\ref{sec:stoch} for the VaR and the CVaR and for a risk level of $\beta:=0.9$ and  a confidence of $1-\delta:=0.95$. The results are shown in table \ref{Tab:UUVRisks_simAndReal}, along with the VaR and CVaR values from \eqref{eq:uuvsystemlin_2} for ease of comparison. The controllers which exhibit higher risk on the linear simulator also exhibit higher risk on the real-time physics engine for both VaR and CVaR, supporting the claims from Section \ref{sec:risk_gap}. This offers empirical evidence that systems which exhibit lower robustness risk in simulation will also exhibit lower robustness risk in the real world.


%UUV case study overview:




%We have a high fidelity model of a UUV in ROS-Gazebo. In the simulator, a UUV operates via heading-speed-depth commands. A bunch of simulation data was collected and a 4th order linearized model of the UUV was obtained via SysID. This model maps HSD commands to the heading-speed-depth of the UUV. Then, reinforcement learning was used to learn a controller for the UUV to follow a pipeline along some offset. This controller was then verified on the linearized model using Verisig.

%We want to use data collected from the linearized model to compute risk bounds for the system for a range of NN based controllers. Then we want to run these controllers on the actual simulator to see how they perform in a more realistic environment. In particular, we aim to show that controllers which are more robust on the linearized model are also more robust on the actual model. 

%The table below shows the var and cvar results for our experiments for different safety range parameters used to train the NN controllers.

\begin{table*}[h]
\caption{UUV risks for a real-time physics engine and a linear simulator for specification \ref{eq:UUVspec}.}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline \specialcell{Safety \\ Range} & \specialcell{Linear \\ Simulator VaR} & \specialcell{Real-Time Physics \\ Engine VaR} & \specialcell{Linear \\ Simulator CVaR} & \specialcell{Real-Time Physics \\ Engine CVaR} \\ \hline
    10 & -10.1215 & -7.9380 & -7.0261 & -4.3691 \\ \hline
    15 & -1.8944 & 5.0788 & 2.3087 & 13.1208 \\ \hline
    30 & -8.2857 & -6.0316 & -5.2708 & 8.7808 \\ \hline
    50 & -10.0697 & -8.3995 & -7.3678 & -5.4930 \\
    \hline
    \end{tabular}
    \label{Tab:UUVRisks_simAndReal}
\end{table*}



%\begin{table*}[h]
%\caption{UUV risks for a high-fidelity simulator and a linearized model for the always safe specification.}
%    \centering
%    \begin{tabular}{|c|c|c|c|c|}
%    \hline Safety Range & Linear Model VaR & Simulation VaR & Linear Model CVaR & Simulation CVaR  \\ \hline
%    10 & -10.081558712502733 & -7.894395070282689 & -7.018185402480389 & -4.369071314298114 \\ \hline
%    15 & -1.894381976464869 & 5.078759635452745 & 2.3086623530430073 & 13.120824002217459 \\ \hline
%    30 & -8.285720602680037 & -5.8562478139734235 & -5.270781390235433 & 81.65188007331035 \\ \hline
%    50 & -10.028407645407007 & -8.36976298396543 & -7.362237771578118 & -5.342417627238612 \\
%    \hline
%    \end{tabular}
%    \label{Tab:UUVRisks_always}
%\end{table*}


Next, we varied the risk level $\beta$  for the VaR and CVaR metrics. These $\beta$ values control how much or little of the tail gets considered in the risk. Larger values only consider the extremes of the tails. Figures \ref{fig:uuvVaRsManyBetas} and \ref{fig:uuvCVaRsManyBetas} show the VaR and CVaR values, respectively, for both the linear simulator and real-time physics engine and different controllers for the specification given in \ref{eq:UUVspec}. In both figures, each controller gets its own color, and risks on the linear simulator are dots, while risks on the real-time physics engine are stars. These figures both show that controllers which exhibit low risk values on the linear simulator also exhibit low risk values on the real-time physics engine and vice versa, and are hence in line with the results in Section \ref{sec:risk_gap}.


% linear model vars
\begin{figure}
\centering
\includegraphics[scale=0.5]{document/figures/vars_over_50_implies_under_50_10_seconds_and_under_10_implies_over_10_10_seconds_diffBetas.png}
\caption{Value-at-Risks (VaRs) for the STL robustness under the specification in \ref{eq:UUVspec} of the 4 different controllers on both UUV models for varied $\beta$ parameters.}
\label{fig:uuvVaRsManyBetas}
\end{figure}


% linear model cvars
\begin{figure}
\centering
\includegraphics[scale=0.5]{document/figures/cvars_over_50_implies_under_50_10_seconds_and_under_10_implies_over_10_10_seconds_diffBetas.png}
\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness under the specification in \ref{eq:UUVspec} of the 4 different controllers on both UUV models for varied $\beta$ parameters.}
\label{fig:uuvCVaRsManyBetas}
\end{figure}






==> chapter/case_studies_risk_verification.tex <==
\section{Case Studies: Risk Verification}

In this section we introduce the case studies considered in this paper and use the risk verification framework to solve Problem \ref{ref:prob1}.


\subsection{F1/10}
\label{sec:F1TenthCaseStudy1}

Our first case study concerns an F1/10 car driving through a hallway with occasional turns. The car is equipped with a LiDAR system for sensing the distances to the hallway. The car must travel through the hallway without colliding into any walls, which is captured with the following constraint function:
\begin{align}\label{eq:F10spec}
    c(x(t),t):= d(x(t)) > d_{w}
\end{align}
where $d(x(t))$ is the distance of the car to the nearest wall at time $t$ and $d_w$ is the minimum allowed distance from the car to the wall.

We used a standard bicycle model as the model of the car. The LiDAR model consisted of noisy range values and a fixed probability of a LiDAR ray randomly getting dropped before each trial.\footnote{A common issue with using LiDAR is that the rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We refer to this as a 'dropped' ray.}
%The specification for the car is that it never collides with the walls of the hallway, which is given in equation \eqref{eq:F10spec}.
Equation \eqref{eq:f1tenthsystemsimlidar} shows the F1-10th with simulated LiDAR written in the form of \eqref{eq:system}. The state is $X = \begin{bmatrix} x & y & v & \theta \end{bmatrix}^T$, where $x$ and $y$ are the car's position, $v$ is the car's velocity, and $\theta$ is the car's heading. The $f$ dynamics function represents a kinematic bicycle model. For more information, see \cite{ivanov2020}. The SiMLiDAR function is the simulated LiDAR model.
\begin{subequations}\label{eq:f1tenthsystemsimlidar}
\begin{align}
    X(t+1)&=f(X(t),\text{DNN}(Y(t))), \; X(0)=X_0\\
    Y(t)&=\text{SiMLiDAR}(X(t)),
\end{align}
\end{subequations}


Next, we used the system in \eqref{eq:f1tenthsystemsimlidar} to train 6 different NN controllers for navigating the car through the hallway, taking LiDAR rays as input and giving steering commands as output. Three of the NNs were trained using the aforementioned TD3 algorithm and the other three were trained using the Deep Deterministic Policy Gradient (DDPG) algorithm \cite{Lillicrap2016ContinuousC}. The reward function used a very large penalty for the car hitting the wall, a small penalty on the magnitude of NN control actions and a small reward for every step the NN took in the simulation environment. Each NN consisted of 2 tanh layers, each of width either 64 or 128 neurons.

We then generated 50000 traces for each of the 6 NNs we trained to guide the F1/10 car through a hallway with a right-hand turn. From these data, we computed the VaR and CVaR risks for each of the controllers using a single risk level of $\beta:=0.9$ and confidence of $1-\delta:=0.95$, which are shown in table \ref{Tab:f1tenthRisks_sim}.


% Table using Rado's controller names
%\begin{table*}[h]
%\caption{F1Tenth VaR values for different LiDAR models under the specification given in \ref{eq:F10spec}.}
%    \centering
%    \begin{tabular}{|c|c|c|c|}
%    \hline Controller Name & Simulated Model VaR & Simulated Model CVaR & Color in Figures  \\ \hline
%    DDPG L21 64x64 C1 & 0.10504042335550173 & 0.13919955860754463 & Black \\ \hline
%    TD3 L21 64x64 C1 & 0.0775641451480904 & 0.11075125542103648 & Red \\ \hline
%    DDPG L21 128x128 C3 & 0.14830549017245062 & 0.18917863635329304 & Green \\ \hline
%    DDPG L21 64x64 C3 & 0.01652110165931031 & 0.08047481958748509 & Blue\\ \hline
%    TD3 L21 128x128 C3 & 0.03684385835564885 & 0.07457605792985965 & Magenta\\ \hline
%    TD3 L21 64x64 C3 & 0.02998700825514189 & 0.06404603055746741 & Cyan \\
%    \hline
%    \end{tabular}
%    \label{Tab:f1tenthRisks_sim}
%\end{table*}

% Table ordered controller names
\begin{table*}[h]
\caption{F1/10 VaR and CVaR values for NN controllers for a simulated LiDAR model under the specification given in \ref{eq:F10spec}.}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline Controller Name & Controller Type & Simulated Model VaR & Simulated Model CVaR  \\ \hline
    1 & DDPG 64x64 & 0.1050 & 0.1392 \\ \hline
    2 & TD3 64x64 & 0.0776 & 0.1108 \\ \hline
    3 & DDPG 128x128 & 0.1483 & 0.1892 \\ \hline
    4 & DDPG 64x64 & 0.0165 & 0.0805 \\ \hline
    5 & TD3 128x128 & 0.0368 & 0.0746 \\ \hline
    6 & TD3 64x64 & 0.0230 & 0.0640 \\
    \hline
    \end{tabular}
    \label{Tab:f1tenthRisks_sim}
\end{table*}





Controllers $4$ and $6$ offers the most robust performance and controllers $1$ and $3$ offer the least robust performance.


This analysis was applied to the simulated system, whereas we are interested in computing risk bounds for the 'real' system. So we next bound the differences in STL robustness risk values between the simulated and real systems.

%We used a standard bicycle model as the model of the car for performing the RL. Our LiDAR model consisted of noisy range values and a fixed probability of a LiDAR randomly getting dropped before each trial.\footnote{A common issue with using LiDAR is that the rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We refer to this as a 'dropped' ray.} The specification for the car is that it never collides with the walls of the hallway, which is given in equation \eqref{eq:F10spec}. %We then ran 50000 trials of each controller navigating through a hallway with a right hand turn. 








%% UUV case study

\subsection{Unmanned Underwater Vehicle (UUV)}
\label{sec:UUVlin}
%\textcolor{red}{General suggestion: I would suggest to use the terminology ``real-time physics engine'' for the gazebo simulator and ``linear simulator'' for the simulations based on the linear model throughout this section to align more with the terminology used before.}

\begin{figure}[ht!]
\centering
\includegraphics[scale=0.25]{document/figures/uuv/uuv_figure_topdown.png}
\caption{The UUV operating environment, both on paper and in the high fidelity physics engine. The pipelines are both shown in blue.}
\label{fig:uuv_fig}
\end{figure}


The UUV is tasked with following alongside a pipeline on the seafloor and using a side-scan sonar system to capture and inspect the pipeline, as shown in Figure \ref{fig:uuv_fig}. As the sonar works best in a certain range of distances from the pipeline, we consider the following requirement in STL that expresses expeditiousness: \textcolor{red}{STL hasn't been introduced yet...}
%\begin{align} \label{eq:UUVspec}
%    \Phi_{UUV}:= &G (d<d_{u} \lor F_{[0,t_{UUV}]} d<d_{u}) \land \\
%    &G (d>d_{l} \lor F_{[0,t_{UUV}]} d>d_{l}) \nonumber
%\end{align}
\begin{align} \label{eq:UUVspec}
    \Phi_{UUV}:= &G \left[d<d_l \implies F_{[0,t_{UUV}]} \left(d \geq d_l \right) \right] \land \\
    &G \left[d>d_u \implies F_{[0,t_{UUV}]} \left(d \leq d_u \right) \right] \nonumber
\end{align}
%\textcolor{red}{1) Use STL terminology from background section, $F$ instead of $\square$, 2) use implication operator instead of disjunction re-formulation for better understanding - only few people are aware of the re-formulation.}
where $d$ is the UUV's distance to the pipeline in the plane, $d_u$ and $d_l$ are the upper and lower distances to the pipe which the UUV must lie within and $t_{UUV}$ is the amount of time in which the UUV is allowed to leave this distance range.\footnote{For example, the UUV may need to avoid obstacles, in which case it is allowed to lose the pipe for a small period of time.}



We consider a high-fidelity UUV model based on the ROS-Gazebo real-time physics engine presented in \cite{Manhaes2016}. As gathering data on real-time systems is time-consuming, we view this model as the perturbed system in \eqref{eq:system_real} and we will instead derive a linearized model corresponding to \eqref{eq:system} next that we can use to collect data more efficiently. \footnote{In the end, however, we will collect data from both systems to support the claims made in Section \ref{sec:risk_gap} with respect to the risk gap between the systems in \eqref{eq:system} and \eqref{eq:system_real}.}

The linearization process is as follows. The UUV uses a pre-existing low level controller to drive the system to a specified heading, speed and depth. The desired heading, speed, depth commands are generated by a separate, high-level controller\footnote{These are the controllers we will synthesize and verify.}.  The goal of the linearization is to make the low level controllers and UUV physics appear linear to the high-level controller.  
Using data from the real-time physics engine, we identified a 4-th order linearized model of the UUV, which takes as input heading, speed, and depth commands (from the high-level controller) and outputs the actual heading, speed, and depth of the UUV. Note that by knowing the UUV's initial location and keeping track of the heading, speed, and depth over time one can compute the UUV's exact position and heading over time.
 


%The linearization process is as follows. The UUV in question uses PID controllers to drive the system to a specified heading, speed and depth. \textcolor{red}{1) I guess heading, speed and depth are the states $X$? Is there no $x$ and $y$ coordinates? Otherwise I don't see how $d$ above is defined. 2) Do I understand it correctly that the PID is only used for obtaining the linearized model? It may be confusing to have two controller, i.e., PID and NN. 3) What are the outputs of the function $u$, i.e, the inputs of the system?}. Using data from this simulator, we identified a 4-th order linearized model \textcolor{red}{We need to emphasize that this corresponds to (3).}  of the UUV \textcolor{red}{linearized around what?}, which takes as input heading, speed, and depth commands and outputs the actual heading, speed, and depth of the UUV \textcolor{red}{I think I'm not entirely following}. 
 
%The equations in \eqref{eq:uuvsystemphys} show the real-time physics engine UUV dynamics. In this case, $Y(t) = \begin{bmatrix} d \\ \theta \end{bmatrix}$ is the distance and heading of the UUV with respect to the pipeline being tracked. The dynamics $f$ and state $X(t)$ are internal to the real-time physics engine, so we keep them general due to space constraints. The SSS function stands for side scan sonar, which is what the UUV uses to detect and track the pipeline. Finally, the DNN function is our DNN controller for the UUV.
%\begin{subequations}\label{eq:uuvsystemphys}
%\begin{align}
%    \overline{X}(t+1)&=f(\overline{X}(t),\text{DNN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
%    \overline{Y}(t)&=\text{SSS}(\overline{X}(t)),
%\end{align}
%\end{subequations}


The equations in \eqref{eq:uuvsystemlin} show the dynamics of the linear simulator of the UUV. Here we have replaced the original dynamics $f$ with the linearized dynamics $f_{lin}$. The linearization also reduces the number of internal UUV states; so we have $\overline{X} = \begin{bmatrix} x_{uuv} & y_{uuv} & \theta_{uuv} &  v_{uuv} & d_{uuv} \end{bmatrix} ^{T}$, which contains the 2-D position, heading, speed and depth of the UUV, respectively. The $V$ term represents the linearization error of the system. Note that there is no measurement error term $W$, since the linearization does not affect the UUV sonar.
\begin{subequations}\label{eq:uuvsystemlin}
\begin{align}
    X(t+1)&=f_{lin}(C(t),\text{DNN}(Y(t))), \; X(0)=X_0\\
    Y(t)&=\text{SSS}(X(t))
\end{align}
\end{subequations}


%In order to get equations \eqref{eq:uuvsystemphys} and \eqref{eq:uuvsystemlin} to resemble equations \eqref{eq:system} and \eqref{eq:system_real}, we rewrite \eqref{eq:uuvsystemphys} as
%\begin{subequations}\label{eq:uuvsystemphyserr}
%\begin{align}
%    \overline{X}(t+1)&=f_{lin}(\overline{X}(t),\text{DNN}(\overline{Y}(t)))+V(\overline{X}(t),\cdot),  \; \overline{X}(0)=X_0,\\
%    \overline{Y}(t)&=\text{SSS}(\overline{X}(t)),
%\end{align}
%\end{subequations}

%So we have replaced the real-time physics engine as the linear simulator plus some linearization error term $V(\overline{X}(t),\cdot)$.

Next, we used the linearized system in \eqref{eq:uuvsystemlin} to train DNN controllers to satisfy the objective in \eqref{eq:UUVspec} via RL.
%Our ultimate goal is to verify DNN controllers that have been trained for these systems and with the objective in \eqref{eq:UUVspec}.
In particular, we  used the Twin Delayed Deep Deterministic Policy Gradients (TD3) algorithm \cite{Fujimoto2018} to train 4 NN controllers for guiding the UUV alongside a pipeline on the seafloor. The reward function for the RL used 4 additive terms. The first term gave a small penalty for each simulation step. The next gave a penalty for the magnitude of the commanded change in heading from the controller. The third gave a penalty for the difference between the UUV's distance to the pipeline and the desired distance to the pipeline. The final term adds a very large penalty if the UUV's distance to the pipe gets outside some safe interval. The size of the safe interval is what we altered for training the controllers. 
%using different reward functions in the RL \textcolor{red}{Give a short hint what exactly is different, and what the reward function is.}. 
Each NN consisted of 2 tanh layers, each of width 32.

To now verify these DNN controllers, each of them was used to generate 5000 runs of the linear simulator 
%and 300 runs of the real-time physics engine,
each corresponding to 3 minutes of data per run.  Finally, the STL robustness risk of the STL specification in \eqref{eq:UUVspec}  is estimated as explained in Section ~\ref{sec:stoch} for the VaR and the CVaR and for a risk level of $\beta:=0.9$ and  a confidence of $1-\delta:=0.95$. The results are shown in table \ref{Tab:UUVRisks_linsim}. 
%The controllers which exhibit higher risk on the linear simulator also exhibit higher risk on the real-time physics engine for both VaR and CVaR, supporting the claims from Section \ref{sec:risk_gap}. 
%\textcolor{red}{I believe that we here have to quantifiy a little more the differences between these systems. As I don't fully understand the linearization yet, this is sth we should discuss.} 
%This offers empirical evidence that systems which exhibit lower robustness risk in simulation will also exhibit lower robustness risk in the real world.


%UUV case study overview:




%We have a high fidelity model of a UUV in ROS-Gazebo. In the simulator, a UUV operates via heading-speed-depth commands. A bunch of simulation data was collected and a 4th order linearized model of the UUV was obtained via SysID. This model maps HSD commands to the heading-speed-depth of the UUV. Then, reinforcement learning was used to learn a controller for the UUV to follow a pipeline along some offset. This controller was then verified on the linearized model using Verisig.

%We want to use data collected from the linearized model to compute risk bounds for the system for a range of NN based controllers. Then we want to run these controllers on the actual simulator to see how they perform in a more realistic environment. In particular, we aim to show that controllers which are more robust on the linearized model are also more robust on the actual model. 

%The table below shows the var and cvar results for our experiments for different safety range parameters used to train the NN controllers.

\begin{table*}[h]
\caption{UUV risks for a real-time physics engine and a linear simulator for specification \ref{eq:UUVspec}.}
    \centering
    \begin{tabular}{|c|c|c|}
    \hline \specialcell{Safety Range} & \specialcell{Linear Simulator VaR} & \specialcell{Linear Simulator CVaR} \\ \hline
    10 & -10.1215 &  -7.0261  \\ \hline
    15 & -1.8944  & 2.3087  \\ \hline
    30 & -8.2857  & -5.2708  \\ \hline
    50 & -10.0697  & -7.3678  \\
    \hline
    \end{tabular}
    \label{Tab:UUVRisks_linsim}
\end{table*}



%\begin{table*}[h]
%\caption{UUV risks for a high-fidelity simulator and a linearized model for the always safe specification.}
%    \centering
%    \begin{tabular}{|c|c|c|c|c|}
%    \hline Safety Range & Linear Model VaR & Simulation VaR & Linear Model CVaR & Simulation CVaR  \\ \hline
%    10 & -10.081558712502733 & -7.894395070282689 & -7.018185402480389 & -4.369071314298114 \\ \hline
%    15 & -1.894381976464869 & 5.078759635452745 & 2.3086623530430073 & 13.120824002217459 \\ \hline
%    30 & -8.285720602680037 & -5.8562478139734235 & -5.270781390235433 & 81.65188007331035 \\ \hline
%    50 & -10.028407645407007 & -8.36976298396543 & -7.362237771578118 & -5.342417627238612 \\
%    \hline
%    \end{tabular}
%    \label{Tab:UUVRisks_always}
%\end{table*}


%Next, we varied the risk level $\beta$  for the VaR and CVaR metrics. These $\beta$ values control how much or little of the tail gets considered in the risk. Larger values only consider the extremes of the tails. Figures \ref{fig:uuvVaRsManyBetas} and \ref{fig:uuvCVaRsManyBetas} show the VaR and CVaR values, respectively, for both the linear simulator and real-time physics engine and different controllers for the specification given in \ref{eq:UUVspec}. In both figures, each controller gets its own color, and risks on the linear simulator are dots, while risks on the real-time physics engine are stars. These figures both show that controllers which exhibit low risk values on the linear simulator also exhibit low risk values on the real-time physics engine and vice versa, and are hence in line with the results in Section \ref{sec:risk_gap}.


% linear model vars used in paper
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_over_50_implies_under_50_10_seconds_and_under_10_implies_over_10_10_seconds_diffBetas.png}
%\caption{Value-at-Risks (VaRs) for the STL robustness under the specification in \ref{eq:UUVspec} of the 4 different controllers on both UUV models for varied $\beta$ parameters.}
%\label{fig:uuvVaRsManyBetas}
%\end{figure}


% linear model cvars used in paper
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_over_50_implies_under_50_10_seconds_and_under_10_implies_over_10_10_seconds_diffBetas.png}
%\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness under the specification in \ref{eq:UUVspec} of the 4 different controllers on both UUV models for varied $\beta$ parameters.}
%\label{fig:uuvCVaRsManyBetas}
%\end{figure}







==> chapter/main_1.tex <==
\section{Risk Verification}
\label{risskk}

In this section, we present a solution to Problem \ref{ref:prob1} and present already one of our two case studies, which is an F1/10 car navigating through a hallway, as shown in Figure \ref{fig:f110_fig}. 
\begin{figure}[ht!]
\centering
\includegraphics[scale=0.5]{document/figures/f1Tenth/f1TenthFig_1.PNG}
\caption{The F1/10 operating environment. The grey dashed lines on the left represent LiDAR rays and the blue curve represents a safe path through the hallway.}
\label{fig:f110_fig}
\end{figure}


\subsection{Estimating an Upper Bound of the Robustness Risk}
As the system in~\eqref{eq:system} defines a stochastic process, Problem~\ref{ref:prob1} can  be solved using frameworks as presented in \cite{lindemann2021stl} \textcolor{red}{(cite more than just [5])}. In this paper, we particularly use the commonly studied risk measures of the value-at-risk and the conditional value-at-risk. We estimate an upper bound of the robustness risk $R(-\rho^c(X))$ from $N$ observed realizations $X^1,\hdots,X^N$ of the stochastic process $X$. Let us, for convenience, first define the random variable 
\begin{align*}
    Z:=-\rho^c(X).
\end{align*}
For further convenience, let us define the tuple
\begin{align*}
    \mathcal{Z}:=(Z^1,\hdots,Z^N)
\end{align*}
where $Z^i:=-\rho^c(X^i,t)$.


\emph{Value-at-Risk (VaR):}  For a risk level of $\beta\in(0,1)$, the VaR of $Z$ is given by
\begin{align*}
VaR_\beta(Z):= \inf\{\alpha\in\mathbb{R}|F_{Z}(\alpha)\ge \beta\}
\end{align*}
where we recall that $F_{Z}(\alpha)$ denotes the CDF of $Z$. To estimate $F_{Z}(\alpha)$, define the empirical CDF 
\begin{align*}
\widehat{F}(\alpha,\mathcal{Z}):=\frac{1}{N}\sum_{i=1}^N \mathbb{I}(Z^i\le \alpha)
\end{align*}
where $\mathbb{I}$ denotes the indicator function. From the empirical CDF, the empirical quantile function of $Z$ is defined as follows:
\begin{align*}
    \widehat{Q}^Z(\tau) = \text{inf} \left\{ x \in \mathbb{R} : \tau \leq \widehat{F}(x,\mathcal{Z}) \right\}
\end{align*}

Next, define the constant
\begin{align*}
    c_N(\delta) = \sqrt{\frac{1}{2N} \text{log} \frac{\pi^2 N^2}{3 \delta}}
\end{align*}

Leveraging quantile estimation results from \cite{Szrnyi2015}, it follows that:

\begin{proposition}\label{prop:quantile}
    Let $\delta \in (0,1)$ be a probability threshold and $\beta \in (0,1)$ be a risk level. The following holds with probability at least $1-\delta$: For all $N \geq 1$:
    \begin{align*}
        VaR_{\beta}(Z) \leq \widehat{Q}(\beta + c_N(\delta))
    \end{align*}
\end{proposition}

%It follows that
%\begin{align*}
%    VaR_{\beta}(Z) \leq \widehat{Q}(\beta + c_N(\delta))
%\end{align*}
%with probabiilty at least $\delta$.


%Let $\delta\in(0,1)$ be a probability threshold. We calculate an upper bound of $VaR_\beta(Z)$ as
%\begin{align*}
%\overline{VaR}_\beta(\mathcal{Z},\delta)&:=\inf\Big\{\alpha\in \overline{\mathbb{R}}|\widehat{F}(\alpha,\mathcal{Z})-\sqrt{\frac{\log(2/\delta)}{2N}}\ge \beta\Big\}.
%\end{align*}


%\begin{proposition}\label{prop:2}
%    Let $\delta\in(0,1)$ be a probability threshold and $\beta\in(0,1)$ be a risk level. Let $\overline{VaR}_\beta(\mathcal{Z},\delta)$  be based on $\mathcal{Z}$ that are $N$ independent copies of $Z$. With probability of at least $1-\delta$, it holds that
%	\begin{align*}
%	 VaR_\beta(Z)\le \overline{VaR}_\beta(\mathcal{Z},\delta).
%	\end{align*}
%\end{proposition}


%For our experiments, we use a quantile estimation from \cite{Szrnyi2015}, which we restate below. The empirical quantile function of $Z$ is defined as follows:

%\begin{align*}
%    \widehat{Q}^Z(\tau) = \text{inf} \left\{ x \in \mathbb{R} : \tau \leq \widehat{F}(x,\mathcal{Z}) \right\}
%\end{align*}

%Next, define the constant

%\begin{align*}
%    c_N(\delta) = \sqrt{\frac{1}{2N} \text{log} \frac{\pi^2 N^2}{3 \delta}}
%\end{align*}


%\begin{proposition}\label{prop:quantile}
%    Fix some $1 \leq k \leq K$ and $\delta \in (0,1)$. The following holds with probability at least $1-\delta$: For all $N \geq 1$ and for every $0 \leq \tau \leq 1$:
%    \begin{align*}
%        Q(\tau) \leq \widehat{Q}(\tau + c_N(\delta))
%    \end{align*}
%\end{proposition}




\emph{Conditional Value-at-Risk (CVaR):} For a risk level of $\beta\in(0,1)$, the CVaR of $Z$ is given by
\begin{align*}
	    CVaR_\beta(Z):=\inf_{\alpha \in {\mathbb{R}}} \; \alpha+(1-\beta)^{-1}E([Z-\alpha]^+)
\end{align*} 
	where $[Z-\alpha]^+:=\max(Z-\alpha,0)$. For estimating  $CVaR_\beta(Z)$ from data $\mathcal{Z}$, we focus here on the case where the random variable $Z=-\rho^\phi(X,t)$ has bounded support (for a fixed $t$) and leverage results from \cite{wang2010deviation}. \textcolor{red}{Missing citation here.} In particular, we assume that $P(Z\in[a,b])=1$. Note that $Z$ has bounded support when $\rho^\phi(X,t)$ is bounded, which can be achieved  either by construction of $\phi$ or by clipping off $\rho^\phi(X,t)$ outside the interval $[a,b]$. 
	%Let now
	%\begin{align*}
	%    \widehat{CVaR}_\beta(\mathcal{Z}):=\inf_{\alpha\in\textcolor{red}{\overline{\mathbb{R}}}}\; \alpha+(N(1-\beta))^{-1}\sum_{i=1}^N[Z^i-\alpha]^+
	%\end{align*}
	%be the empirical estimate of $CVaR_\beta(Z)$. We can now calculate an upper bound of $CVaR_\beta(Z)$ as
	%\begin{align*}
	%    &\overline{CVaR}_\beta(\mathcal{Z},\delta):=\widehat{CVaR}_\beta(\mathcal{Z})+\sqrt{\frac{11\log(6/\delta)}{N(1-\beta)}}(b-a).
	%\end{align*}
	%\begin{proposition}\label{prop:3}
	%    Let $\delta\in(0,1)$ be a probability threshold and $\beta\in(0,1)$ be a risk level. Assume that $P(Z\in[a,b])=1$. Let $\overline{CVaR}_\beta(\mathcal{Z},\delta)$ and $\underline{CVaR}_\beta(\mathcal{Z},\delta)$ be based on $\mathcal{Z}$ that are $N$ independent copies of $Z$. With probability of at least $1-\delta$, it holds that
	%\begin{align*}
  %CVaR_\beta(Z)\le \overline{CVaR}_\beta(\mathcal{Z},\delta).
	%\end{align*}
	%\end{proposition}

By leveraging results from \cite{thomas2019concentration}, we can compute an upper bound of $CVaR_{\beta}(Z)$ as follows:

%We use the result from \cite{thomas2019concentration} for computing CVaR in the experiments. For convenience, we restate a portion of their main results.

\begin{proposition}
    Let $\delta\in(0,1)$ be a probability threshold and $\beta\in(0,1)$ be a risk level. Assume that $P(Z\in[a,b])=1$. Let $Z^1,\hdots,Z^n$ be $n$ independent copies of random variable $Z$. Then
    \begin{align*}
        Pr \left( CVaR_{\beta}(Z) \leq O_{n+1} - \frac{1}{\beta} \sum_{i=1}^{n} (O_{i+1} - O_{i})  \left( \frac{i}{n} - \sqrt{\frac{ln(1/\delta)}{2n}} - (1-\beta) \right)^+ \right) \geq 1-\delta
    \end{align*}
    where $O_1,\hdots,O_n$ are the order statistics (i.e. $Z^1,\hdots,Z^n$ sorted in ascending order), $Z^{n+1} = b$, and $x^+ := max\{0,x\}$ for all $x\in \mathbb{R}$.
\end{proposition}



\subsection{Case Studies}
\label{sec:F1TenthCaseStudy1}

Our first case study concerns an F1/10 car driving through a hallway with occasional turns. The car is equipped with a LiDAR system for sensing the distances to the hallway. The car must travel through the hallway without colliding into any walls, which is captured with the following constraint function:
\begin{align}\label{eq:F10spec}
    c(x(t),t):= d(x(t)) > d_{w}
\end{align}
where $d(x(t))$ is the distance of the car to the nearest wall at time $t$ and $d_w$ is the minimum allowed distance from the car to the wall.

We used a standard bicycle model as the model of the car. The LiDAR model consisted of noisy range values and a fixed probability of a LiDAR ray randomly getting dropped before each trial.\footnote{A common issue with using LiDAR is that the rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We refer to this as a 'dropped' ray.}
%The specification for the car is that it never collides with the walls of the hallway, which is given in equation \eqref{eq:F10spec}.
Equation \eqref{eq:f1tenthsystemsimlidar} shows the F1-10th with simulated LiDAR written in the form of \eqref{eq:system}. The state is $X = \begin{bmatrix} x & y & v & \theta \end{bmatrix}^T$, where $x$ and $y$ are the car's position, $v$ is the car's velocity, and $\theta$ is the car's heading. The $f$ dynamics function represents a kinematic bicycle model. For more information, see \cite{ivanov2020}. The SiMLiDAR function is the simulated LiDAR model.
\begin{subequations}\label{eq:f1tenthsystemsimlidar}
\begin{align}
    X(t+1)&=f(X(t),\text{DNN}(Y(t))), \; X(0)=X_0\\
    Y(t)&=\text{SiMLiDAR}(X(t)),
\end{align}
\end{subequations}


We trained 6 different NN controllers for navigating the car through the hallway, taking LiDAR rays as input and giving steering commands as output. Then we generated 50000 traces for each of the 6 NNs we trained to guide the F1/10 car through a hallway with a right-hand turn. From these data, we computed the VaR and CVaR risks for each of the controllers using a single risk level of $\beta:=0.9$ and confidence of $1-\delta:=0.95$, which are shown in table \ref{Tab:f1tenthRisks_sim}.


% Table using Rado's controller names
%\begin{table*}[h]
%\caption{F1Tenth VaR values for different LiDAR models under the specification given in \ref{eq:F10spec}.}
%    \centering
%    \begin{tabular}{|c|c|c|c|}
%    \hline Controller Name & Simulated Model VaR & Simulated Model CVaR & Color in Figures  \\ \hline
%    DDPG L21 64x64 C1 & 0.10504042335550173 & 0.13919955860754463 & Black \\ \hline
%    TD3 L21 64x64 C1 & 0.0775641451480904 & 0.11075125542103648 & Red \\ \hline
%    DDPG L21 128x128 C3 & 0.14830549017245062 & 0.18917863635329304 & Green \\ \hline
%    DDPG L21 64x64 C3 & 0.01652110165931031 & 0.08047481958748509 & Blue\\ \hline
%    TD3 L21 128x128 C3 & 0.03684385835564885 & 0.07457605792985965 & Magenta\\ \hline
%    TD3 L21 64x64 C3 & 0.02998700825514189 & 0.06404603055746741 & Cyan \\
%    \hline
%    \end{tabular}
%    \label{Tab:f1tenthRisks_sim}
%\end{table*}

% Table ordered controller names
\begin{table*}[h]
\caption{F1/10 VaR and CVaR values for NN controllers for a simulated LiDAR model under the specification given in \ref{eq:F10spec}.}
    \centering
    \begin{tabular}{|c|c|c|}
    \hline Controller Name & Simulated Model VaR & Simulated Model CVaR  \\ \hline
    1 & 0.1050 & 0.1392 \\ \hline
    2 & 0.0776 & 0.1108 \\ \hline
    3 & 0.1483 & 0.1892 \\ \hline
    4 & 0.0165 & 0.0805 \\ \hline
    5 & 0.0368 & 0.0746 \\ \hline
    6 & 0.0230 & 0.0640 \\
    \hline
    \end{tabular}
    \label{Tab:f1tenthRisks_sim}
\end{table*}





Controllers $4$ and $6$ offers the most robust performance and controllers $1$ and $3$ offer the least robust performance.


This analysis was applied to the simulated system, whereas we are interested in computing risk bounds for the 'real' system. So we next bound the differences in STL robustness risk values between the simulated and real systems.

%We used a standard bicycle model as the model of the car for performing the RL. Our LiDAR model consisted of noisy range values and a fixed probability of a LiDAR randomly getting dropped before each trial.\footnote{A common issue with using LiDAR is that the rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We refer to this as a 'dropped' ray.} The specification for the car is that it never collides with the walls of the hallway, which is given in equation \eqref{eq:F10spec}. %We then ran 50000 trials of each controller navigating through a hallway with a right hand turn. 




==> chapter/main_2.tex <==







\section{The Risk Gap}
\label{sec:risk_gap}



At time $t$, and without any further assumption on $u$, we can upper bound the error $\|\overline{X}(t,\omega)- X(t,\omega)\|$ between the system trajectories of the nominal system \eqref{eq:system} and the perturbed system \eqref{eq:system_real} for each realization $\omega\in\Omega$ by the function 
%\textcolor{red}{I think we should derive $\Delta(t+1)$ and not just provide the result}
\begin{align*}
    \Delta(t+1):=L_{f,1}\Delta(t)+L_{f,2}L_u(L_g\Delta(t)+w^*)+v^*
\end{align*}
where $\Delta(0):=0$ and where $L_{f,1}$ and $L_{f,2}$ are the Lipschitz constants of the first and second arguments of $f$, $L_g$ is the Lipschitz constant of $g$, and $v^*$ and $w^*$ are calculated as
\begin{align*}
    v^*:=\max_{v\in D_v}\|v\| \,\;\text{ and } \,\; w^*:=\max_{w\in D_w}\|w\|.
\end{align*}

This can be shown to hold as follows:
\begin{align*}
    \Delta(t+1) &= \| \overline{X}(t,\omega) - X(t,\omega) \| \\
    &= \| f(\overline{X}(t,\omega),u(\overline{Y}(t))) + V(t,\omega) - f(X(t,\omega),u(Y(t))) \| \\
    &= \| f(\overline{X}(t,\omega),u(g(\overline{X}(t,\omega)) + W(t,\omega)) + V(t,\omega) - f(X(t,\omega),u(g(X(t,\omega))) \| \\
    & \leq  L_{f,1} \| \overline{X}(t,\omega) - X(t,\omega) \|  + L_{f,2} \| u(g(\overline{X}(t,\omega)) + W(t,\omega)) - u(g(X(t,\omega))) \| + v^* \\
    &\leq L_{f,1} \Delta(t) + L_{f,2} L_{u} \|  g(\overline{X}(t,\omega)) - g(X(t,\omega)) + W(t,\omega) \| + v^*\\
    & \leq L_{f,1} \Delta(t) + L_{f,2} L_{u} (L_{g} \| \overline{X}(t,\omega) - X(t,\omega) \| + w^*) + v^* \\
    &\leq L_{f,1} \Delta(t) + L_{f,2} L_{u} (L_{g} \Delta(t) + w^*) + v^*
\end{align*}
In other words, it holds that
\begin{align*}
    \|\overline{X}(t,\omega)- X(t,\omega)\|\le \Delta(t).
\end{align*}
Note that the error bound $\Delta(t)$ grows unbounded with  time $t$. We can avoid this when putting an additional assumption on $u$, i.e., when $u$ is such that the system in \eqref{eq:system_real} is incrementally input-to-state stable (see e.g., \cite{tran2016incremental}). In particular, let $D:=(V,W)$ and $D_D:=D_v\times D_w$, then the system \eqref{eq:system_real} is incrementally input-to-state stable for every $X_0(\omega)$ if there exists a function $\gamma \in \mathcal{K}_{\infty}$ such that 
\begin{align*}
    \|\overline{X}(t,\omega;D_1)- \overline{X}(t,\omega;D_2)\|\le  \gamma(\sup_{d_1,d_2\in D} \|d_1-d_2\|)
\end{align*}
where $\overline{X}(t,\omega;D_i)$ is the solution to \eqref{eq:system_real} but where $D$ is replaced with a stochastic process $D_i:\mathbb{N}\times\Omega\to D_D$. While this may seem like a stringent assumption on the system, learning controllers that exhibit iISS or similar stability properties is an active area of research \cite{tu2021closing,Havens2021}.


%\textcolor{red}{Remark on how realistic this assumption is and cite related literature, like Nik's paper. Also, https://arxiv.org/pdf/2103.12945.pdf}


%Consider the discrete time, deterministic, non-linear system

%\begin{align}\label{eq:iISSsystem}
%    x(t+1) = f(x(t),u(t)), \; \; \; x(t) \in \mathbb{R}^n, \; u(t) \in \mathbb{R}^m, \; \; \; t \in \mathcal{Z}_{\geq 0}
%\end{align}

%where $f : \mathbb{R}^n \times \mathbb{R}^m$ is continuous, $f(0,0)=0$, and $u : \mathcal{Z}_{\geq 0} \rightarrow \mathbb{R}^m$ denotes an input sequence. Denote $x : \mathcal{Z}_{\geq 0} \times \mathbb{R}^n \times \mathbb{R}^m \rightarrow \mathbb{R}^n$ as the solution to system \ref{eq:iISSsystem} from an initial condition $\xi \in \mathbb{R}^n$ and subject to input sequence $u$.

%\begin{definition} \label{def:iiss}
%A discrete time system is incrementally Input-To-State Stable (iISS) if there exist functions $\beta \in \mathcal{K}\mathcal{L}$, and $\gamma \in \mathcal{K}_{\infty}$ such that
%\begin{align}
%    \left\lVert x(t,\xi_1,u_1) - x(t,\xi_2,u_2) \right\rVert \leq \beta(\left\lVert \xi_1 - \xi_2\right\rVert,t) + \gamma(\left \lVert u_1 - u_2 \right \rVert_{\infty})
%\end{align}
%\textcolor{red}{Introduce notation $x(t,\xi_1,w_1)$. Let's use $d$ to denote disturbances (instead of $w$)?}

%\end{definition}

As the origin is contained within $D_D$ by assumption, it follows in this case that the error bound between the system trajectories of the nominal system \eqref{eq:system} and the perturbed system \eqref{eq:system_real} are independent of $t$, i.e., that
\begin{align*}
    \|\overline{X}(t,\omega)- X(t,\omega)\|\le  \gamma(\sup_{d_1,d_2\in D} \|d_1-d_2\|).
\end{align*}


Note that this shows an incentive to learn incrementally input-to-state stable control laws such as in \cite{tu2021closing,boffi2021regret}. For convenience, let $\Gamma:=\gamma(\sup_{d_1,d_2\in D} \|d_1-d_2\|)$. Let us next provide an example of an incrementally input-to-state-stable system.
\begin{example}
%\textcolor{red}{We may want to include a perception map (or Kalman filter?) here as well...}
Consider the stochastic system as in \eqref{eq:system} defined by
\begin{align*}
    A:=\mathcal{I}_2\otimes \begin{bmatrix}
    1 & 0.5  \\
    0 & 1  
    \end{bmatrix} \;  B :=\mathcal{I}_2\otimes \begin{bmatrix}
    0.125  \\
    0.5
    \end{bmatrix} \;
    C := \mathcal{I}_2\otimes \mathcal{I}_2 \nonumber
\end{align*}
%\textcolor{red}{Let's use $t$ in here as a time index?}

Next, we design a linear feedback controller $K$ to stabilizes the system via the well known linear quadratic regulator (LQR):
\begin{align*}
    K = \mathcal{I}_2 \otimes \begin{bmatrix}
    0.6514 & 1.3142
    \end{bmatrix}
\end{align*}

%The stabilized system now becomes
%\begin{align} \label{eq:exSystem}
%    A_{cl} = \mathcal{I}_2 \otimes \begin{bmatrix} 0.9186 & 0.3357 \\ -0.3257 & 0.3429
%    \end{bmatrix} \;  B :=\mathcal{I}_2\otimes \begin{bmatrix}
%    0.125  \\
%    0.5
%    \end{bmatrix} \;
%    C := \mathcal{I}_2\otimes \mathcal{I}_2
%\end{align}


The stabilized system now becomes
\begin{align} \label{eq:exSystem}
    A_{cl} = \mathcal{I}_2 \otimes \begin{bmatrix} 0.9186 & 0.3357 \\ -0.3257 & 0.3429
    \end{bmatrix}
\end{align}

First, we prove that \eqref{eq:exSystem} is incrementally input to state stable iISS.


%Recall that a discrete time system is globally incrementally Input-To-State Statble (iISS) if there exist functions $\beta \in \mathcal{K}\mathcal{L}$, and $\sigma \in \mathcal{K}_{\infty}$ such that
%\begin{align}
%    \left| x(k,\xi_1,w_1) - x(k,\xi_2,w_2) \right| \leq \beta(\left| \xi_1 - \xi_2\right|,k) + \sigma(\left \lVert w_1 - w_2 \right \rVert_{\infty})
%\end{align}


For a discrete linear system with initial state $x_0$, the state after $t$ time steps under additive disturbances $d[i],i=0\hdots,t$ is %when given input $u[i],i=0,\hdots,t$ is
\begin{align}
    x_{d}[t] = A_{cl}^t x_0 + \sum_{i=0}^{t-1} A_{cl}^{t-i-1} d[i]
\end{align}

Now we consider two traces of the system, one with disturbance $d_1$ and the other with disturbance $d_2$ and both starting at initial state $x_0$. It follows that
\begin{align}
    \left| x_{d_1}[t] - x_{d_2}[t] \right| &= \left| A_{cl}^t x_0 + \sum_{i=0}^{t-1} A_{cl}^{t-i-1} d_1[i] - A_{cl}^t x_0 + \sum_{i=0}^{t-1} A^{t-i-1} d_2[i] \right| \\
    &= \left| \sum_{i=0}^{t-1} A_{cl}^{t-i-1} (d_1[i]-d_2[i]) \right| \\
    &\leq \sum_{i=0}^{\infty} \left \lVert A_{cl} \right \rVert^i \left \lVert d_1-d_2\right \rVert_{\infty}
\end{align}
The last line follows from the sub-multiplicativity of matrix norms.
    

Our system is stable, hence $A_{cl}$ has spectral radius less than 1. Thus $\sum_{i=0}^{\infty} \left \lVert A_{cl} \right \rVert^i = \frac{1}{1-\left \lVert A_{cl} \right \rVert}$ and $\gamma(\| d \|)=\frac{1}{1- \left \lVert A_{cl} \right \rVert} \| d \|$ clearly satisfies the definition of iISS, concluding the proof.


Now consider a perturbed version of the stabilized system in \eqref{eq:exSystem}, where the perturbations are modeled as in \eqref{eq:system_real}. Let $v^*=0.5$ and $w^*=0.1$. Since our system is iISS, the trace differences between the nominal and perturbed systems, assuming the initial conditions are equivalent, are bounded by 
\begin{align*}
     \|\overline{X}(t,\omega)- X(t,\omega)\| &\leq \gamma ( 2v^* + 2w^* ) \\
    &= \frac{1.2}{1- \left \lVert A_{cl} \right \rVert}
\end{align*}
\end{example}



\subsection{Quantifying the Risk Gap}

%\textcolor{red}{Remove STL business from here and put it into the STL section instead. Then rewrite this section for the constraint function $c$.}

So far, we have quantified how close trajectories of  the nominal system \eqref{eq:system} and the perturbed system \eqref{eq:system_real} will be. Our next goal is to quantify how this impacts the STL robustness.


\begin{lemma}\label{lemma:1_c}
 Consider the stochastic control systems in  \eqref{eq:system} and \eqref{eq:system_real} under a controller $u$. Let $c:\mathbb{R}^n\times \mathbb{T}\to \mathbb{R}$ be a measurable constraint function with $T:=\max \mathbb{T}$ being bounded. Then it  holds that
 \begin{align}\label{eq:phi_inequ_c}
  \rho^c(X(\cdot,\omega))-\Delta(T)\le \rho^c(\overline{X}(\cdot,\omega))
\end{align} for each realization $\omega\in\Omega$. 

\begin{proof}
For convenience, let $\overline{x}:=\overline{X}(\cdot,\omega)$ and $x:=X(\cdot,\omega)$. First, recall that the robustness function $\rho^c(x)$ for the constraint function $c$ is defined as
\begin{align*}
    \rho^c(x):=\inf_{t\in\mathbb{T}} \, \text{Dist}^c(x(t),t)
\end{align*}
where the signed distance $\text{Dist}^c(x(t),t)$ is
\begin{align*}
    \text{Dist}^c(x(t),t):=\begin{cases}
    \inf_{x'\in \text{cl}(O^{\neg c}(t))} \|x(t)-x'\| &\text{if } c(x(t),t)\ge 0\\
    -\inf_{x'\in \text{cl}(O^c(t))} \|x(t)-x'\| &\text{otherwise. }
    \end{cases}
\end{align*}

%\begin{align*}
%    \rho^{\mu}(x,t)& := \begin{cases} \text{dist}^{\neg\mu}(x,t) &\text{if } x\in \mathcal{L}^\mu(t)\\
%	-\text{dist}^{\mu}(x,t) &\text{otherwise,}
%	\end{cases}
%\end{align*}


It holds that $\inf_{x'\in \text{cl}(O^{\neg c}(t))} \|x(t)-x'\|$ and $\inf_{x'\in \text{cl}(O^c(t))} \|x(t)-x'\|$ are Lipschitz continuous functions with Lipschitz constant one, see for instance \cite[Chapter 3]{munkres1975prentice}. Accordingly, it can be shown that $\text{Dist}^c(x(t),t)$ is Lipschitz continuous in its first argument with Lipschitz constant one. From this, we have for time $t$ that  $|\text{Dist}^c(x(t),t)-\text{Dist}^c(\overline{x}(t),t)| \le \|x(t)-\overline{x}(t)\|\le \Delta(t)$. By the definition of $\rho^c$, we consequently have that $|\rho^c(x)-\rho^c(\overline{x})|\le \max_{t\in\mathbb{T}} \Delta(t)=\Delta(T)$. Finally, it follows that $ \rho^c(x)\ge \rho^c(\overline{x})- \Delta(T)$.
\end{proof}
\end{lemma}

The previous bound may be quite conservative as $\Delta(t)$ grows with increasing time $t$. As remarked before, such conservatism can be avoided when the controller $u$ is incrementally input-to-state stable.
\begin{lemma}\label{lemma:2_c}
 Consider the stochastic control systems in  \eqref{eq:system} and \eqref{eq:system_real} under a controller $u$ that renders the system \eqref{eq:system_real} incrementally input-to-state stable for every $X_0(\omega)$. Let $c:\mathbb{R}^n\times \mathbb{T}\to \mathbb{R}$ be a measurable constraint function. Then it  holds that
 \begin{align}\label{eq:phi_inequ__c}
  \rho^c(X(\cdot,\omega))-\Gamma\le \rho^c(\overline{X}(\cdot,\omega))
\end{align} for each realization $\omega\in\Omega$. 

\begin{proof}
The proof follows similar arguments as the proof of Lemma \ref{lemma:1}, but now simply  replacing $\Delta(t)$ by $\Gamma$.
\end{proof}
\end{lemma}



Now that we have quantified in Lemmas \ref{lemma:1_c} and \ref{lemma:2_c} how close the STL robustness of the systems in \eqref{eq:system} and \eqref{eq:system_real} will be, we are ready to quantify the risk gap. Under the same conditions as in Lemma \ref{lemma:1_c}, we derive the following bound.
\begin{theorem}\label{thm:1_c}
Let the conditions of Lemma \ref{lemma:1_c} hold and let the risk measure $R$ be monotone and translationally invariant. Then it holds that 
\begin{align*}
    R(-\rho^c(\overline{X}))\le R(-\rho^c(X))+\Delta(T).
\end{align*}

\begin{proof} 
 By \eqref{eq:phi_inequ_c} and since the risk measure $R$ is monotone, it follows that $R(-\rho^c(\overline{X}))\le R(-\rho^c(X)+\Delta(T))$. Since $R$ is additionally translationally invariant, it further holds that $R(-\rho^c(X)+\Delta(T))=R(-\rho^c(X))+\Delta(T)$ so that $R(-\rho^c(\overline{X}))\le R(-\rho^c(X))+\Delta(T)$, which concludes the proof.
\end{proof}
\end{theorem}

Under the same conditions as in Lemma \ref{lemma:2_c}, we next derive the following bound that is independent of $t$.
\begin{theorem}\label{thm:2_c}
Let the conditions of Lemma \ref{lemma:2_c} hold and let the risk measure $R$ be monotone and translationally invariant. Then it holds that 
\begin{align*}
    R(-\rho^c(\overline{X}))\le R(-\rho^c(X))+\Gamma.
\end{align*}

\begin{proof} 
The proof follows in analogy to the proof of Theorem \ref{thm:1_c}, but now using Lemma \ref{lemma:2_c} instead of Lemma \ref{lemma:1_c}.
\end{proof}
\end{theorem}



 We can now use the risk gap to compare controllers to address Problem \ref{ref:prob2}.



\begin{corollary}
Let the conditions of Theorem \ref{thm:1_c} hold. Assume that $R(-\rho^c(X_{u_1}))\le R(-\rho^c(X_{u_2}))-c$ for two control laws $u_1$ and $u_2$. Then it holds that $R(-\rho^c(\overline{X}_{u_1}))\le R(-\rho^c(\overline{X}_{u_2}))$ if $2\Delta(T)\le c$.
\end{corollary}

\begin{corollary}
Let the conditions of Theorem \ref{thm:2_c} hold. Assume that $R(-\rho^c(X_{u_1}))\le R(-\rho^c(X_{u_2}))-c$ for two control laws $u_1$ and $u_2$. Then it holds that $R(-\rho^c(\overline{X}_{u_1}))\le R(-\rho^c(\overline{X}_{u_2}))$ if $2\Gamma\le c$.
\end{corollary}


%%%%%%%%%
% STL SECTION
%%%%%%%%%

\section{Signal Temporal Logic}
\label{sec:STL}
Signal temporal logic \cite{maler2004monitoring} is based on signals, and in this paper in particular on discrete-time signals $x:\mathbb{N}\to\mathbb{R}^n$. The atomic elements of STL are predicates that are functions $\mu:\mathbb{R}^n\to\mathbb{B}$. Let now $M$ be a set of such predicates $\mu$ and let us associate an observation map $O^\mu\subseteq \mathbb{R}^n$ with $\mu$. The observation map $O^\mu$ indicates regions within the state space where $\mu$ is true, i.e.,
\begin{align*}
O^\mu:=\mu^{-1}(\top)
\end{align*}
where $\mu^{-1}(\top)$ denotes the inverse image of $\top$ under $\mu$.
\begin{remark}\label{rem:1}
For convenience, the predicate $\mu$ is often defined via a predicate function $h:\mathbb{R}^n\to\mathbb{R}$ so that
\begin{align*}
\mu(\zeta):=\begin{cases}
\top & \text{if } h(\zeta)\ge 0\\
\bot &\text{otherwise}
\end{cases}
\end{align*}
for $\zeta\in\mathbb{R}^n$. In this case, we have  $O^\mu=\{\zeta\in\mathbb{R}^n|h(\zeta)\ge 0\}$.
\end{remark}



For $\mu\in M$, the syntax of STL, also referred to as the grammar of STL, is recursively defined as 
\begin{align}\label{eq:full_STL}
\phi \; ::= \; \top \; | \; \mu \; | \;  \neg \phi \; | \; \phi' \wedge \phi'' \; | \; \phi'  U_I \phi'' \; | \; \phi' \underline{U}_I \phi'' \,
\end{align}
where $\phi'$ and $\phi''$ are STL formulas. The meanings of the negation and conjunction operators $\neg$ and $\wedge$ are `not' and  `and'. The future until operator $\phi' {U}_I \phi''$ encodes that $\phi'$ is true until $\phi''$ becomes true within the time interval $I\subseteq \mathbb{R}_{\ge 0}$, while $\underline{U}_I$ is the past until-operator. Also define the operators
\begin{align*}
F_I\phi&:=\top U_I \phi &\text{ (future eventually operator)},\\
\underline{F}_I\phi&:=\top \underline{U}_I \phi &\text{ (past eventually operator)},\\
G_I\phi&:=\neg F_I\neg \phi &\text{ (future always operator)},\\
\underline{G}_I\phi&:=\neg \underline{F}_I\neg \phi &\text{ (past always operator),}\\
\phi' \vee \phi''&:=\neg(\neg\phi' \wedge \neg\phi'') &\text{ (disjunction operator)}.
\end{align*}
The future eventually operator $F_I\phi$ encodes that $\phi$ holds in the future at least once  within the interval $I$, while the future always operator $G_I\phi$ encodes that $\phi$ holds in the future at all times  within the interval $I$. The past  eventually and past always operators follow similar reasoning, while the disjunction operator $\vee$ encodes 'or'.  We provide the semantics of STL \cite{maler2004monitoring} that determine whether or not a signal $x$ satisfies the STL formula $\phi$ at time $t$ in Appendix \ref{app:STL_sem}. An STL formula $\phi$ is bounded if all time intervals $I$ in $\phi$ are bounded. Each bounded STL formula $\phi$ has a future formula length $L_f^\phi$ that defines how long a signal has to be in order to  be able to say whether or not it satisfies $\phi$, see Appendix \ref{app:STL_sem} for a formal statement. 
 
\emph{Robustness.} One may especially be interested in the robustness by which a signal $x$ satisfies the STL formula $\phi$ at time $t$.  For this purpose, the authors in \cite{fainekos2009robustness} introduce the robustness degree and in particular the function $\text{dist}^{\neg\phi}:\mathfrak{F}(\mathbb{N},\mathbb{R}^n)\times\mathbb{N}\to\mathbb{R}_{\ge 0}$. Intuitively, $\text{dist}^{\neg\phi}(x,t)$ measures the distance of the signal $x$ to the set of signals that violate $\phi$ at time $t$ (see Appendix \ref{app:STL} for a formal definition). It holds that $\text{dist}^{\neg\phi}(x,t)=0$ indicates that $x$ violates or marginally satisfies $\phi$, while $\text{dist}^{\neg\phi}(x,t)>0$ indicates that $x$ satisfies $\phi$. In fact, larger values of $\text{dist}^{\neg\phi}(x,t)$ indicate that $\phi$ is satisfied more robustly.  Unfortunately, $\text{dist}^{\neg\phi}(x,t)$ is in general difficult to calculate. The  authors in \cite{fainekos2009robustness} introduce the \emph{robust semantics} $\rho^\phi:\mathfrak{F}(\mathbb{N},\mathbb{R}^n)\times \mathbb{N}\to \mathbb{R}$ as a tractable but more conservative robustness estimate, i.e., it holds that $\rho^{\phi}(x,t)\le \text{dist}^{\neg\phi}(x,t)$ \cite[Theorems 28]{fainekos2009robustness}. For a formal definition, we refer to Definition \ref{def:quantitative_semantics} in Appendix \ref{app:STL}.  
 
 
\begin{example}\label{ex1}
Consider a scenario in which a robot operates in a hospital environment. The robot needs to perform two time-critical sequential delivery tasks in regions $A$ and $B$ while avoiding areas $C$ and $D$ in which humans operate.  In particular, we consider the STL formula 
\begin{align}\label{ex:1_formula}
    \phi:=G_{[0,3]}\neg (\mu_{C} \wedge \mu_{D}) \wedge F_{[1,2]}(\mu_{A} \wedge F_{[0,1]}\mu_{B}).
\end{align}
To define  $\mu_A$, $\mu_B$, $\mu_C$, and $\mu_D$, let $a$, $b$, $c$, and $d$ denote the midpoints of the regions $A$, $B$, $C$, and $D$ as
\begin{align*}
    a&:=\begin{bmatrix}
        4 & 5
    \end{bmatrix}^\mathbb{N}
     \hspace{0.5cm} b:=\begin{bmatrix}
        7 & 2
    \end{bmatrix}^\mathbb{N}\\
     c&:=\begin{bmatrix}
        2 & 3
    \end{bmatrix}^\mathbb{N}
     \hspace{0.5cm}d:=\begin{bmatrix}
        6 & 4
    \end{bmatrix}.^\mathbb{N}
\end{align*}
Also let the state $x(t)\in\mathbb{R}^{10}$ at time $t$ be
\begin{align*}
    x(t):=\begin{bmatrix}r(t) & a & b& c& d \end{bmatrix}^\mathbb{N}
\end{align*} 
where $r$ is the robot position at time $t$. The predicates $\mu_A$, $\mu_B$, $\mu_C$, and $\mu_D$ are now described by the observation maps
\begin{align*}
    O^{\mu_A}&:=\{x\in\mathbb{R}^{10}|\|r-a\|_\infty\le 0.5\},\\
    O^{\mu_B}&:=\{x\in\mathbb{R}^{10}|\|r-b\|_2\le 0.7\},\\
    O^{\mu_C}&:=\{x\in\mathbb{R}^{10}|\|r-c\|_\infty\le 0.5\},\\
    O^{\mu_D}&:=\{x\in\mathbb{R}^{10}|\|r-d\|_2\le 0.7\}.
\end{align*}
where $\|\cdot\|_2$ is the Euclidean and $\|\cdot\|_\infty$ is the infinity norm. In Fig. \ref{ex:1_figure}, six different robot trajectories $r_1$-$r_6$ are displayed. It can be seen that the signal $x_1$ that corresponds to $r_1$ violates $\phi$, while $x_2$-$x_6$ satisfy $\phi$. In particular, we obtain $\rho^\phi(x_1,0)=-0.15$, $\rho^\phi(x_2,0)=0$, and $\rho^\phi(x_i,0)=0.25$ for all $i\in\{3,\hdots,6\}$. The reason for $x_1$ having negative robustness lies in $r_1$ intersecting with the region $D$. Marginal robustness of $x_2$ is explained as $r_2$ only marginally avoids the region $D$ while all other trajectories avoid the region $D$ robustly.
\begin{figure}
\centering
\includegraphics[scale=0.5]{figures/ex1.png}
\caption{Shown are six robot trajectories $r_1$-$r_6$ along with four regions $A$, $B$, $C$, and $D$. The specification given in \eqref{ex:1_formula} is violated by $r_1$ and satisfied by $r_2$-$r_6$. Furthermore, $r_2$ only marginally satisfies  $\phi$, while $r_3$-$r_6$ satisfy $\phi$ robustly.}
\label{ex:1_figure}
\end{figure}
\end{example}




The risk of the stochastic process $X$ not satisfying $\phi$ robustly, called the ``STL robustness risk'' \cite{lindemann2021stl}, is defined next.
 \begin{definition}
 	Given an STL formula $\phi$ and a stochastic process $X:\mathbb{N}\times\Omega\to\mathbb{R}^n$, the risk of $X$ not satisfying $\phi$ robustly at time $t$ is defined as $R(-\text{dist}^{\neg\phi}(X,t))$.
 \end{definition}
 
As remarked in Section \ref{sec:STL}, the function $\text{dist}^{\neg\phi}$ is in general hard to calculate and work with. In \cite[Thm. 3]{lindemann2021stl}, we have presented conditions on $R$ under which $R(-\text{dist}^{\neg\phi}(X,t))\le R(-\rho^\phi(X,t))$, i.e., $R(-\rho^\phi(X,t))$ is more risk-averse than $R(-\text{dist}^{\neg\phi}(X,t))$ and may instead be used. We refer to $R(-\rho^\phi(X,t))$ as the approximate STL robustness risk.
\begin{proposition}\label{thm:3}
	Let $R$ be a monotone risk measure. Then it holds that $R(-\text{dist}^{\neg\phi}(X,t))\le R(-\rho^\phi(X,t))$.
\end{proposition}

%\textcolor{red}{Instead of interpreting an STL specifications $\phi$ over deterministic signals, we will interpret $\phi$ over stochastic processes. }



\subsection{Quantifying the Risk Gap: STL}

So far, we have quantified how differences between trajectories of the nominal system \eqref{eq:system} and the perturbed system \eqref{eq:system_real} impact the robustness of our system for properties specified as constraint functions $c(x(t),t)$. We now quantify how differences between the aforementioned trajectories impact the STL robustness.

%So far, we have quantified how close trajectories of the nominal system \eqref{eq:system} and the perturbed system \eqref{eq:system_real} will be. Our next goal is to quantify how this impacts the STL robustness.


\begin{lemma}\label{lemma:1}
 Consider the stochastic control systems in  \eqref{eq:system} and \eqref{eq:system_real} under a controller $u$. Let  $\phi$ be a bounded STL formula in positive normal form  with formula length $L_f^\phi$. For $t\in\mathbb{N}$, it  holds that
 \begin{align}\label{eq:phi_inequ}
  \rho^\phi(X(\cdot,\omega),t)-\Delta(t+L_f^\phi)\le \rho^\phi(\overline{X}(\cdot,\omega),t))
\end{align} for each realization $\omega\in\Omega$. 

\begin{proof}
For convenience, let $\overline{x}:=\overline{X}(\cdot,\omega)$ and $x:=X(\cdot,\omega)$. The proof follows inductively on the structure of $\phi$ and without considering the case of negations as $\phi$ is assumed to be in positive normal form.

\emph{Predicates. } First recall the STL robust semantics for predicates defined in Appendix \ref{app:STL} as
\begin{align*}
    \rho^{\mu}(x,t)& := \begin{cases} \text{dist}^{\neg\mu}(x,t) &\text{if } x\in \mathcal{L}^\mu(t)\\
	-\text{dist}^{\mu}(x,t) &\text{otherwise,}
	\end{cases}
\end{align*}
and note that
\begin{align*}
	\text{dist}^{\mu}(x,t)= \bar{d}\big(x(t),\text{cl}(O^\mu)\big):=\inf_{x'\in \text{cl}(O^\mu)} d(x(t),x').
	\end{align*} 
	according to \cite[Lemma 57]{fainekos2009robustness}. It further holds that $\bar{d}$ is a Lipschitz continuous function with Lipschitz constant one, see for instance \cite[Chapter 3]{munkres1975prentice}. Accordingly, it can be shown that $\rho^{\mu}(x,t)$ is Lipschitz continuous in its first argument with Lipschitz constant one. From this, we have for each predicate $\mu_i$ and for each time $t'\le t+L_f^\phi$ that  $|\rho^{\mu_i}(x,t')-\rho^{\mu_i}(\overline{x},t')| \le \|x(t')-\overline{x}(t')\|\le \Delta(t')\le \Delta(t+L_f^\phi)$ where the last inequality follows by closeness of solutions and since $\Delta(t')\le \Delta(t+L_f^\phi)$ for $t'\le t+L_f^\phi$. Consequently, we have that $ \rho^{\mu_i}(\overline{x},t')\ge \rho^{\mu_i}(x,t)- \Delta(t+L_f^\phi)$ for $t'\le t+L_f^\phi$.

\emph{Conjunctions. } For conjunctions $\phi'\wedge\phi''$ and by the induction assumption, it holds that $ \rho^{\phi'}(\overline{x},t')\ge \rho^{\phi'}(x,t')- \Delta(t+L_f^\phi)$ and $ \rho^{\phi''}(\overline{x},t')\ge \rho^{\phi''}(x,t')- \Delta(t+L_f^\phi)$ for $t'\le t+L_f^{\phi}-L_f^{\phi'\wedge\phi''}$. Now, it follows that
\begin{align*}
    \rho^{\phi'\wedge \phi''}(\overline{x},t')&=\min(\rho^{\phi'}(\overline{x},t'),\rho^{\phi'}(\overline{x},t'))\\
    &\ge \min(\rho^{\phi'}(x,t'),\rho^{\phi''}(x,t'))- \Delta(t+L_f^\phi)\\
    &=\rho^{\phi'\wedge \phi''}(x,t')- \Delta(t+L_f^\phi).
\end{align*}

\emph{Future and past Until. } Using the induction assumption and a similar reasoning as for conjunctions, it follows that $ \rho^{\phi'U_I \phi''}(\overline{x},t')\ge \rho^{\phi'U_I \phi''}(x,t')- \Delta(t+L_f^\phi) \; $ for $t'\le t+L_f^\phi- L_f^{\phi'U_I \phi''} \; $ and $\;  \rho^{\phi'\underline{U}_I \phi''}(\overline{x},t')\ge \rho^{\phi'\underline{U}_I \phi''}(x,t')- \Delta(t+L_f^\phi)\; $ for $\; t'\le t+L_f^\phi- L_f^{\phi'\underline{U}_I \phi''}$. 


It can hence be concluded that \eqref{eq:phi_inequ} holds.
\end{proof}
\end{lemma}

The previous bound may be quite conservative as $\Delta(t+L_f^\phi)$ grows with increasing time $t$ and formula length $L_f^\phi$. As remarked before, such conservatism can be avoided when the controller $u$ is incrementally input-to-state stable.
\begin{lemma}\label{lemma:2}
 Consider the stochastic control systems in  \eqref{eq:system} and \eqref{eq:system_real} under a controller $u$ that renders the system \eqref{eq:system_real} incrementally input-to-state stable for every $X_0(\omega)$. Let $\phi$ be an STL formula. For $t\in\mathbb{N}$, it holds that 
\begin{align}\label{eq:phi_inequ_}
  \rho^\phi(X(\cdot,\omega),t)-\Gamma\le \rho^\phi(\overline{X}(\cdot,\omega),t))
\end{align}
for each realization $\omega\in\Omega$.

\begin{proof}
The proof follows similar arguments as the proof of Lemma \ref{lemma:1}, but now simply  replacing $\Delta(t+L_f^\phi)$ by $\Gamma$.
\end{proof}
\end{lemma}


Now that we have quantified in Lemmas \ref{lemma:1} and \ref{lemma:2} how close the STL robustness of the systems in \eqref{eq:system} and \eqref{eq:system_real} will be, we are ready to quantify the risk gap. Under the same conditions as in Lemma \ref{lemma:1}, we derive the following bound.
\begin{theorem}\label{thm:1}
Let the conditions of Lemma \ref{lemma:1} hold and let the risk measure $R$ be monotone and translationally invariant. Then it holds that 
\begin{align*}
    R(-\rho^\phi(\overline{X},t))\le R(-\rho^\phi(X,t))+\Delta(t+L_f^\phi).
\end{align*}

\begin{proof} 
 By \eqref{eq:phi_inequ} and since the risk measure $R$ is monotone, it follows that $R(-\rho^\phi(\overline{X},t))\le R(-\rho^\phi(X,t)+\Delta(t+L_f^\phi))$. Since $R$ is additionally translationally invariant, it further holds that $R(-\rho^\phi(X,t)+\Delta(t+L_f^\phi))=R(-\rho^\phi(X,t))+\Delta(t+L_f^\phi)$ so that $R(-\rho^\phi(\overline{X},t))\le R(-\rho^\phi(X,t))+\Delta(t+L_f^\phi)$, which concludes the proof.
\end{proof}
\end{theorem}

Under the same conditions as in Lemma \ref{lemma:2}, we next derive the following bound that is independent of $t$ and the $L_f^\phi$.
\begin{theorem}\label{thm:2}
Let the assumption of Lemma \ref{lemma:2} hold and let the risk measure $R$ be monotone and translationally invariant. Then it holds that 
\begin{align*}
    R(-\rho^\phi(\overline{X},t))\le R(-\rho^\phi(X,t))+\Gamma.
\end{align*}

\begin{proof} 
The proof follows in analogy to the proof of Theorem \ref{thm:1}, but now using Lemma \ref{lemma:2} instead of Lemma \ref{lemma:1}.
\end{proof}
\end{theorem}



While the risk gap may potentially be conservative, we emphasize that it applies to all formulas and a range of systems. We can now use the risk gap to compare controllers.



\begin{corollary}
Let the conditions of Theorem \ref{thm:1} hold. Assume that $R(-\rho^\phi(X_{u_1},t))\le R(-\rho^\phi(X_{u_2},t))-k$ for two control laws $u_1$ and $u_2$. Then it holds that $R(-\rho^\phi(\overline{X}_{u_1},t))\le R(-\rho^\phi(\overline{X}_{u_2},t))$ if $2\Delta(t+L_f^\phi)\le k$.

\begin{proof}
Use Lemma \ref{lemma:1} and Theorem \ref{thm:1}.
\end{proof}
\end{corollary}





==> chapter/problem_statement.tex <==
\section{Problem Statement}
\label{sec:problem_statement}


%Before we formulate the risk verification problem, 
We first give two case studies on which to introduce the high level risk verification problem. The case studies considered in this paper are an F1/10 car in a hallway and a unmanned underwater vehicle (UUV) tracking a pipeline on the seafloor. After the case studies, we introduce the \textcolor{blue}{high level} risk verification \textcolor{blue}{problem}. %\textcolor{red}{Rado: should probably summarize the rest of the section also here. Also, maybe say why we start with the case studies}

\subsection{Case Studies}




\begin{figure}[ht!]
\centering
\includegraphics[scale=0.5]{document/figures/f1Tenth/f1TenthFig_1.PNG}
\caption{The F1/10 operating environment. The grey dashed lines on the left represent LiDAR rays and the blue curve represents a safe path through the hallway.}
\label{fig:f110_fig}
\end{figure}


\textbf{F1/10 car.} Our first case study concerns an F1/10 car \cite{F1/10} driving through a hallway with 90-degree turns, as shown in Figure \ref{fig:f110_fig}. The car is equipped with a LiDAR system for sensing the distances to the hallway. We used a standard bicycle model of the car and a ground truth LiDAR model to model the car in simulation. Given this simple closed-loop simulator setup, we used RL to train NN controllers to safely navigate the car through the hallway. The first question we are interested in is which controller performs best in simulation, i.e., results in the lowest risk. In addition, it has been shown that NN controllers which are verified to be safe in simulation can still show poor performance when evaluated in the real world \cite{ivanov2020}. So if a controller performs well in simulation, what is the risk of it causing the real F1/10 car to crashing into the walls of the hallway?
%\footnote{In \cite{ivanov2020}, the authors showed that controllers which are verified to be safe in simulation can show poor performance when moved to the real world.} 
%\textcolor{red}{(Rado: I think this needs a bit more explanation. Why did we use RL? Why is there any risk if we verified the car is safe? These case studies need to motivate the rest of the paper.)}






\begin{figure}[ht!]
\centering
\includegraphics[scale=0.25]{document/figures/uuv/uuv_figure_topdown.png}
\caption{The UUV operating environment, both on paper and in the high fidelity physics engine. The pipelines are both shown in blue.}
\label{fig:uuv_fig}
\end{figure}

\textbf{UUV.} The second case study concerns a UUV that is tasked with following alongside a pipeline on the seafloor and using a side-scan sonar system to capture and inspect the pipeline, as shown in Figure \ref{fig:uuv_fig}. We consider a high-fidelity UUV model based on the ROS-Gazebo real-time physics engine presented in \cite{Manhaes2016}. As the real-time physics engine is too computationally complex to generate large amounts of data, we fit a partially linearized model of the UUV. Using this model, we use RL to train NN controllers to guide the UUV along the pipe, while keeping an optimal distance for the sonar to accurately inspect the pipe. Once again, we can ask similar questions to the F1/10 case: which NN controller best guides the UUV along the pipe in the modeled environment? What are the risks of these NN controllers not properly guiding the UUV along the pipe in the real-time physics engine? 


\subsection{Problem Formulation}
\label{sec:problem_formulation}

The focus in this paper is on the verification of \emph{stochastic dynamic control systems with NN controllers} in the loop. In particular, we are interested to verify systems in terms of the risk of violating a given specification.  We also show under which conditions an acceptable risk of a system, e.g., a simulator, implies an acceptable risk for a perturbed version of the system, e.g., a real system. %\textcolor{red}{(Rado: this is a bit confusing. Is the simulator the real (complex) thing, or is it an abstraction of the real thing?)}


Consider therefore the stochastic dynamic system
\begin{align}
\begin{split}
    X(t+1)&=f(X(t),u(Y(t))), \; X(0)=X_0\\
    Y(t)&=g(X(t)),
\end{split}
\label{eq:system}
\end{align}
where the Lipschitz continuous functions $f:\mathbb{R}^n\times\mathbb{R}^m\to\mathbb{R}^n$ and $g:\mathbb{R}^n\to\mathbb{R}^p$ describe the system dynamics and the output measurement map, respectively, and where the function $u:\mathbb{R}^p\to\mathbb{R}^m$ is an NN controller. The functions $f$ and $g$ do not need to be known as long as we can draw system trajectories from \eqref{eq:system}. We, however, assume to know the Lipschitz constants of $f$, $g$, and $u$. Note that Lipschitz constants of NN controllers $u$ can be calculated as, for instance, described in \cite{fazlyab2019efficient}.  The initial position $X_0 \in \mathbb{R}^n$ of the system is a random variable so that $X$ defines a stochastic process. We remark that $X_0$ is the only source of randomness in \eqref{eq:system}. This is done for simplicity.

%and without loss of generality. \textcolor{red}{Matthew: A reviewer complained about the 'without loss of generality. Can we concisely argue why this is ok? Rado: I am honestly not sure if it's wlog. Maybe we just say drop the `wlog'?}

%In general, we could also assume that both the system dynamics and the output measurement map are affected by random variables.(\textcolor{red}{Rado: I think this remark is misleading and potentially arguable. Probably better just to bring up the perturbed system here -- the original model can be wrong, so we also considered the perturbed case.})

As seen with the case studies introduced previously, we expect our system to be operating in a different environment from which it was trained (e.g. the UUV controllers were trained on a linearized system and operate in a realistic physics engine). We view such system differences as perturbations. Let us hence consider the perturbed system
\begin{align}
\begin{split}
    \overline{X}(t+1)&=f(\overline{X}(t),u(\overline{Y}(t)))+V(t), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=g(\overline{X}(t))+W(t),
\end{split}
\label{eq:system_real}
\end{align}
where the functions $V:\mathbb{N}\to D_v \subseteq \mathbb{R}^n$ and $W:\mathbb{N}\to D_w \subseteq \mathbb{R}^p$ define stochastic processes that describe modeling errors and disturbances. We assume that the sets $D_v$ and $D_w$ are compact and contain the origin.  In \eqref{eq:system_real}, we consider that the uncertainties $V$ and $W$ enter the dynamics linearly.  Nonlinear effects can also be modelled as long as the system dynamics remain locally Lipschitz continuous in $V$ and $W$. Note also that $V$ and $W$ can be functions of $\overline{X}(t)$, which is however omitted for readability reasons.

%The two problems we are interested in solving are:
%\begin{enumerate}
%    \item \emph{Risk Verification}: Given the stochastic control system in \eqref{eq:system}, a specification it must satisfy and an NN controller, compute the risk of the system robustly satisfying the specification.
%    \item \emph{Risk Gap}: Given the stochastic control system in \eqref{eq:system}, a specification, an NN controller, and the perturbed system in \eqref{eq:system_real}, compute an upper bound on the difference in robustness risks between the two systems when both use the NN controller. In addition, given two controllers and their robustness risks on system \eqref{eq:system}, determine if one controller is guaranteed to have a lower robustness risk on the perturbed system \eqref{eq:system_real}.
%\end{enumerate}

%Given the systems in~\eqref{eq:system} and~\eqref{eq:system_real}, the high-level question is what is the risk of these systems violating some safety specification $c(x(t),t)$, as formalized below. In particular, ML algorithms that synthesize NN controllers $u$ in general provide no formal correctness guarantees for satisfying the specification at hand, especially not for stochastic systems as in \eqref{eq:system}. We hence aim to verify NN controllers in terms of their induced robustness risk.


%\textcolor{red}{Move this somewhere in section 4.2 ...}
%$R(-\rho^c(X))$ (\textcolor{red}{Rado: we haven't defined $\rho$ yet, so probably drop this notation from here.})where the function $R(\cdot)$ is a risk metric as detailed in Section \ref{sec:sol_1}.\footnote{Note here that $\rho^c(X(\cdot,\omega))$ is measurable in $\omega$ so that $\rho^c(X)$ is a random variable. To see this, note first that $\text{Dist}^c(X(t,\omega),t)$ is measurable in $\omega$ for a fixed $t\in\mathbb{T}$ since: 1) the function $c(X(t,\omega))$ is measurable in $\omega$ for a fixed $t\in\mathbb{T}$, 2) the indicator function of a measurable set is measurable, and 3) the distance function to a non-empty set, i.e., $\inf_{x'\in \text{cl}(O^{\neg c}(t))} \|x(t)-x'\|$, is continuous (see e.g., \cite[Chapter 3]{munkres1975prentice}) and hence measurable. Measurability of $\rho^c(X(\cdot,\omega))$ in $\omega$ now follows as the infimum over a countable number of measurable functions is again measurable, see e.g., \cite[Theorem 4.27]{guide2006infinite}. Consequently, $\rho^c(X)$ and hence $-\rho^c(X)$ are random variables so that $R(-\rho^c(X))$ is well defined.}

%When using learning to synthesize controllers there are many training parameters that one can employ. This leads to a situation where a set of controllers gets trained by varying said parameters. So one would like to know: 1) which of these controllers satisfy the specification, and 2) which controller is the best in terms of its robustness. 



%Often enough (\textcolor{red}{Rado: informal}) one ends up with a set of controllers, obtained by varying training parameters, and one would like to know: 1) which of these controllers satisfy the specification, and 2) which controller is the best in terms of its robustness. 


In what follows, we provide an abstract statement of the risk verification problem -- the fully formalized setting is presented in Section~\ref{sec:sol_1}. We consider systems subject to real-time safety constraints. For instance, the F1/10 car needs to avoid colliding with walls at all times. For simplicity, we first express real-time constraints as follows
\begin{align*}
    c(x(t),t)\ge 0 \text{ for all } t\in\mathbb{T}
\end{align*}
where $c:\mathbb{R}^n\times \mathbb{T}\to \mathbb{R}$ is a measurable constraint function (e.g., hyper-planes representing walls in the F1/10 example) and $x:\mathbb{T}\to\mathbb{R}^n$ is a signal \textcolor{blue}{of the system}, e.g., the trajectory of the robot. Later in Section \ref{sec:STL}, we consider signal temporal logic (STL) as a more principled means, i.e., being close to structured English, to express such real-time constraints. 

%\textcolor{red}{Now introduce the idea of robustness}

Next, we consider how robustly system traces satisfy (or violate) the constraint functions. To do so, we first note that $c$ defines a set of safe states, denoted by $O^c(t)$
\begin{align*}
    \textcolor{blue}{O^c(t) := \left\{ x \in \mathbb{R}^n | c(x,t) \geq 0 \right\}.}
\end{align*}
Now given a \textcolor{blue}{signal $x$ and time $t$} we compute the distance from $x(t)$ to the boundary of the safe set $O^c(t)$, which we denote as $\text{Dist}^c(x(t),t)$. 
%\textcolor{blue}{If $x(t) \in O^c(t)$ then $\text{Dist}^c(x(t),t) \geq 0$ and if $x(t) \notin O^c(t)$ then $\text{Dist}^c(x(t),t) < 0$.} 
\textcolor{blue}{Intuitively, this distance represents how close $x(t)$ is to satisfying (or not satisfying) the constraint function $c$ at time $t$. We define the robustness of signal $x$ as the smallest distance to the safe set over time}
\begin{align*}
    \rho^c(x):=\inf_{t\in\mathbb{T}} \, \text{Dist}^c(x(t),t).
\end{align*}
Note that $\rho^c(x(t)) > 0$ implies that $x(t)$ satisfies the specification. Intuitively, this quantifies how much one would need to alter the trace to cause it to violate (or satisfy) the constraint. For example, consider a trace of the F1/10 car where it comes within 1m of colliding with the wall. We would say that this trace has a robustness of 1. Finally, we are interested in computing risk metrics over the robustness $\rho^c(x(t))$, denoted as $R(-\rho^c(X))$. \textcolor{blue}{Commonly used risk metrics are the expected value, the variance, the value-at-risk, or the conditional value-at-risk \cite{rockafellar2000optimization}. We formally introduce risk metrics in Section \ref{sec:stoch} and} safe/unsafe sets, trace distances and robustness values in Section \ref{sec:robustness_risk}.



\begin{comment}

%\textcolor{red}{MC: Move this to background section? Or put at end of this section? It shouldn't go here but not sure where to put it.}
\begin{example}
In the short example from the above introduction, we may particularly consider the constraint function 
\begin{align*}
    c(x(t),t):=\begin{cases}
    1 & \text{for all } t<T_1 \text{ and all } t>T_2\\
    h(x(t)) & \text{for all } t\in [T_1,T_2]
    \end{cases}
\end{align*} 
where $h:\mathbb{R}^n\to \mathbb{R}$ encodes the spatial constraint of the robot being in a designated area. The constraint $c(x(t),t)\ge 0$ is, in this case, equivalent to $h(x(t))\ge 0$ for all $t\in [T_1,T_2]$.
\end{example}

Importantly, we can quantify how robustly a signal $x$ satisfies the constraint $c(x(t),t)\ge 0$. Therefore, let us define the sets \begin{align*}
    O^c(t)&:=\{x\in\mathbb{R}^n| c(x,t)\ge 0\}\\
    O^{\neg c}(t)&:=\{x\in\mathbb{R}^n| c(x,t)< 0\}
\end{align*}
that indicate the part of the state space where $x(t)$ satisfies and violates the constraint $c(x(t),t)\ge 0$, respectively. We can now define the signed distance $\text{Dist}^c:\mathbb{R}^n\times\mathbb{T}\to\mathbb{R}$ from $x(t)$ to the set $O^c(t)$ as
\begin{align*}
    \text{Dist}^c(x(t),t):=\begin{cases}
    \inf_{x'\in \text{cl}(O^{\neg c}(t))} \|x(t)-x'\| &\text{if } c(x(t),t)\ge 0\\
    -\inf_{x'\in \text{cl}(O^c(t))} \|x(t)-x'\| &\text{otherwise }
    \end{cases}
\end{align*}
where cl$(\cdot)$ denotes the closure operation of a set. In words, $\text{Dist}^c(x(t),t)$ denotes how much one would need to alter the value of signal $x$ at time $t$ to have it violate (satisfy) constraint $c(x(t),t)$, provided $x(t)$ already satisfies (violates) the constraint at time $t$. For instance, a value of $\text{Dist}^c(x(t),t)=2$ means that $x(t)$ would need to be altered by at least $2$ in order to violate $c(\cdot, \cdot)$ (and vice versa if $\text{Dist}^c(x(t),t)=-2$).


%\textcolor{red}{Provide some intuition on $\text{Dist}^c(x(t),t)$.} 
Let us next define the \emph{robustness function} $\rho^c:\mathfrak{F}(\mathbb{T},\mathbb{R}^n)\to\mathbb{R}$, where $\mathfrak{F}(\mathbb{T},\mathbb{R}^n)$ denotes the set of all measurable functions mapping from the domain $\mathbb{T}$ into the domain $\mathbb{R}^n$,   as
\begin{align*}
    \rho^c(x):=\inf_{t\in\mathbb{T}} \, \text{Dist}^c(x(t),t).
\end{align*}
Naturally, notice that $\rho^c(x)\ge 0$ implies that the specification is satisfied by $x$, i.e., that $c(x(t),t)\ge 0$ for all $t\in\mathbb{T}$. If $\rho^c(x)>0$, notice further that all signals $x':\mathbb{T}\to\mathbb{R}^n$ that are such that $\|x(t)-x'(t)\|<\rho^c(x)$ for all $t\in\mathbb{T}$ also satisfy the specification, i.e., are such that $\rho^c(x')>0$. In the remainder, we will not evaluate the constraint function $c$ over a deterministic signal $x$, but instead over a stochastic process $X$, i.e., we aim to use $c(X(t,\cdot),t)$.

\end{comment}



\begin{problem}[Risk Verification]\label{ref:prob1}
Assume the stochastic control system in \eqref{eq:system}, in particular we focus on an unmanned underwater vehicle and an F-10th car, and a measurable constraint function $c:\mathbb{R}^n\times \mathbb{T}\to \mathbb{R}$. Assume a set of NN controllers $u_i$ is given. Calculate the robustness risks $R(-\rho^c(X_i))$ for the system in \eqref{eq:system} under each NN controller $u_i$.\footnote{We use the notation $X_i$ to indicate the stochastic trajectory of the system in \eqref{eq:system}  under the NN controller $u_i$.} 
\end{problem}

 To solve Problem \ref{ref:prob1}, we use data sampled from the system \eqref{eq:system}  under the NN controller $u_i$ to obtain an \emph{upper bound} of  $R(-\rho^c(X_i))$ with high probability. We emphasize that we are interested in an upper bound of $R(-\rho^c(X_i))$ to be  risk averse as opposed to being risk neutral by estimating the mean of $R(-\rho^c(X_i))$. Our main goal in Problem \ref{ref:prob1} is to analyze the effect of different risk metrics and different risk levels that can act as a tuning knob between risk averse and risk neutral decision making. We also argue that robustness should be used as a quality measure compared to existing verification techniques that rely on a binary verification answer. 
 

The second problem that we address in this paper is to investigate how the robustness risk $R(-\rho^c(X))$, calculated in Problem~\ref{ref:prob1}, can be used to determine how the NN controllers perform on systems that are different from~\eqref{eq:system}, i.e., how the robustness risk $R(-\rho^c(X))$ can aid in determining if an NN controller is robust enough to be used for a perturbed version of the system as in \eqref{eq:system_real}. 
\begin{remark}
Part of our motivation is that both training and verification of an NN may require a lot of data that can often only be obtained in a simulator. In our solution to Problem \ref{ref:prob1} and to acquire  reliable and accurate estimates of the robustness risk $R(-\rho^c(X))$, we may require large amounts of data. Obtaining data from real physical systems is oftentimes not possible as it may be too time consuming and expensive. Instead, one may want to verify a controller based on data obtained from a simulator, while showing how the robustness risk $R(-\rho^c(X))$ may increase on the real system. 
\end{remark}

%Let us hence consider the perturbed system 
%\begin{subequations}\label{eq:system_real}
%\begin{align}
%    \overline{X}(t+1)&=f(\overline{X}(t),u(\overline{Y}(t)))+V(t,\cdot), \; \overline{X}(0)=X_0\\
%    \overline{Y}(t)&=g(\overline{X}(t))+W(t,\cdot),
%\end{align}
%\end{subequations}
%where the functions $V:\mathbb{N}\times\Omega\to D_v \subseteq \mathbb{R}^n$ and $W:\mathbb{N}\times\Omega\to D_w \subseteq \mathbb{R}^p$ define stochastic processes that describe modeling errors and disturbances. We assume that the sets $D_v$ and $D_w$ are compact and contain the origin.  In \eqref{eq:system_real}, we consider that the uncertainties $V$ and $W$ enter the dynamics linearly.  Nonlinear effects can also be modelled as long as the system dynamics remain locally Lipschitz continuous in $V$ and $W$. Note also that $V$ and $W$ can be functions of $\overline{X}(t)$, which is however omitted for readability reasons.


\textcolor{blue}{Particularly, we are interested to upper bound the \emph{risk verification gap} $R(-\rho^c(\overline{X}))-R(-\rho^c(X))$ in the second problem considered in this paper.}

\begin{problem}[Risk Verification Gap]\label{ref:prob2}
Assume the stochastic control systems in  \eqref{eq:system} and \eqref{eq:system_real} and a measurable constraint function $c:\mathbb{R}^n\times \mathbb{T}\to \mathbb{R}$. 
\begin{enumerate}
    \item \textcolor{blue}{Find a constant $\Delta\in\mathbb{R}$ and conditions on the controller $u$, the risk metric $R$, and the random variables $V$ and $W$ such that the risk verification gap $R(-\rho^c(\overline{X}))-R(-\rho^c(X))$ is upper bounded by $\Delta$.}
    \item Let two NN controllers $u_1$ and $u_2$ be given. If $R(-\rho^c(X_1))\le R(-\rho^c(X_2))$, provide conditions on the controllers $u_1$ and $u_2$, the risk metric $R$, and the random variables $V$ and $W$ such that $R(-\rho^c(\overline{X}_1))\le R(-\rho^c(\overline{X}_2))$.
\end{enumerate}
\end{problem}

While the first part of Problem \ref{ref:prob2} addresses the risk verification gap, the second part of Problem \ref{ref:prob2} asks for conditions so that a controller that has a lower robustness risk on the nominal system \eqref{eq:system} than another controller also has a lower robustness risk on the perturbed system \eqref{eq:system_real}.


\begin{comment}


\subsection{Case Studies}

We now introduce the case studies on which we will solve Problems \ref{ref:prob1} and \ref{ref:prob2}.

\subsubsection{F1/10}
\label{sec:F1TenthCaseStudy1}

\begin{figure}[ht!]
\centering
\includegraphics[scale=0.5]{document/figures/f1Tenth/f1TenthFig_1.PNG}
\caption{The F1/10 operating environment. The grey dashed lines on the left represent LiDAR rays and the blue curve represents a safe path through the hallway.}
\label{fig:f110_fig}
\end{figure}


Our first case study concerns an F1/10 car driving through a hallway with occasional turns, as shown in Figure \ref{fig:f110_fig}. The car is equipped with a LiDAR system for sensing the distances to the hallway.
%The car must travel through the hallway without colliding into any walls.
We used a standard bicycle model as the model of the car. The LiDAR model consisted of noisy range values.

%and a fixed probability of a LiDAR ray randomly getting dropped before each trial.\footnote{A common issue with using LiDAR is that the rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We refer to this as a 'dropped' ray.}
%The specification for the car is that it never collides with the walls of the hallway, which is given in equation \eqref{eq:F10spec}.

Equation \eqref{eq:f1tenthsystemsimlidar} shows the F1-10th with simulated LiDAR written in the form of \eqref{eq:system}. The state is $X = \begin{bmatrix} x & y & v & \theta \end{bmatrix}^T$, where $x$ and $y$ are the car's position, $v$ is the car's velocity, and $\theta$ is the car's heading. The $f$ dynamics function represents a kinematic bicycle model. For more information, see \cite{ivanov2020}. The SiMLiDAR function is the simulated LiDAR model.
\begin{subequations}\label{eq:f1tenthsystemsimlidar}
\begin{align}
    X(t+1)&=f(X(t),\text{NN}(Y(t))), \; X(0)=X_0\\
    Y(t)&=\text{SiMLiDAR}(X(t)),
\end{align}
\end{subequations}


Next, we used the system in \eqref{eq:f1tenthsystemsimlidar} to train 6 different NN controllers for navigating the car through the hallway, taking LiDAR rays as input and giving steering commands as output. Three of the NNs were trained using the aforementioned TD3 algorithm and the other three were trained using the Deep Deterministic Policy Gradient (DDPG) algorithm \cite{Lillicrap2016ContinuousC}. The reward function used a very large penalty for the car hitting the wall, a small penalty on the magnitude of NN control actions and a small reward for every step the NN took in the simulation environment. Each NN consisted of 2 tanh layers, each of width either 64 or 128 neurons.

A common issue with using LiDAR is that the rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We refer to this as a 'dropped' ray. To generate a more realistic LiDAR model to use for testing in simulation, we added a fixed probability of a LiDAR ray randomly getting dropped before each trial. Equation \eqref{eq:f1tenthsystemdroppedraylidar} shows the F1-10th with dropped ray LiDAR model written in the form of \eqref{eq:system}. The dynamics $f$ and state $\overline{X}$ are the same as in \eqref{eq:f1tenthsystemsimlidar}. The DroppedRayLiDAR function is the dropped ray LiDAR model.
\begin{subequations}\label{eq:f1tenthsystemdroppedraylidar}
\begin{align}
    X(t+1)&=f(X(t),\text{NN}(Y(t))), \; X(0)=X_0\\
    Y(t)&=\text{DroppedRayLiDAR}(X(t)),
\end{align}
\end{subequations}

To simulate real-world LiDAR data, we  trained a GAN to approximate LiDAR readings from real-world LiDAR data. The GAN had a deconvoluational NN architecture \cite{radford2016} and was trained using the Wasserstein GAN algorithm \cite{arjovsky2017,gulrajani2017}. The GAN takes in the position and heading of the car and a 10 dimensional (random) seed and outputs an array of 21 LiDAR rays. Equation \eqref{eq:f1tenthsystemganlidar} shows the F1-10th with GAN LiDAR. The dynamics $f$ and state $\overline{X}$ are the same as in \eqref{eq:f1tenthsystemsimlidar}. The GANLiDAR function is the GAN LiDAR model.
\begin{subequations}\label{eq:f1tenthsystemganlidar}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{NN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{GANLiDAR}(\overline{X}(t)),
\end{align}
\end{subequations}

We now rewrite equation \eqref{eq:f1tenthsystemganlidar} to match the form of \eqref{eq:system_real}. The $W$ term accounts for the measurement differences between the dropped ray LiDAR model and the GAN LiDAR model. There is no $V$ term here, since the dynamics of the two system models are equivalent. 
\begin{subequations}\label{eq:f1tenthsystemganlidarerr}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{NN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{DroppedRayLiDAR}(\overline{X}(t)) + W(\overline{X}(t),\cdot),
\end{align}
\end{subequations}
where $W(\overline{X}(t),\cdot)=\text{GaNLiDAR}(\overline{X}(t)) - \text{DroppedRayLiDAR}(X(t))$.



\subsection{Unmanned Underwater Vehicle (UUV)}
\label{sec:UUVCaseStudy1}

\begin{figure}[ht!]
\centering
\includegraphics[scale=0.25]{document/figures/uuv/uuv_figure_topdown.png}
\caption{The UUV operating environment, both on paper and in the high fidelity physics engine. The pipelines are both shown in blue.}
\label{fig:uuv_fig}
\end{figure}


The UUV is tasked with following alongside a pipeline on the seafloor and using a side-scan sonar system to capture and inspect the pipeline, as shown in Figure \ref{fig:uuv_fig}. 
%As the sonar works best in a certain range of distances from the pipeline, we consider the following requirement in STL that expresses expeditiousness: \textcolor{red}{STL hasn't been introduced yet...}

%\begin{align} \label{eq:UUVspec}
%    \Phi_{UUV}:= &G \left[d<d_l \implies F_{[0,t_{UUV}]} \left(d \geq d_l \right) \right] \land \\
%    &G \left[d>d_u \implies F_{[0,t_{UUV}]} \left(d \leq d_u \right) \right] \nonumber
%\end{align}
%where $d$ is the UUV's distance to the pipeline in the plane, $d_u$ and $d_l$ are the upper and lower distances to the pipe which the UUV must lie within and $t_{UUV}$ is the amount of time in which the UUV is allowed to leave this distance range.\footnote{For example, the UUV may need to avoid obstacles, in which case it is allowed to lose the pipe for a small period of time.}



We consider a high-fidelity UUV model based on the ROS-Gazebo real-time physics engine presented in \cite{Manhaes2016}. The equations in \eqref{eq:uuvsystemphys} show the real-time physics engine UUV dynamics. In this case, $Y(t) = \begin{bmatrix} d \\ \theta \end{bmatrix}$ is the distance and heading of the UUV with respect to the pipeline being tracked. The dynamics $f$ and state $X(t)$ are internal to the real-time physics engine, so we keep them general due to space constraints. The SSS function stands for side scan sonar, which is what the UUV uses to detect and track the pipeline. Finally, the NN function is our NN controller for the UUV.
\begin{subequations}\label{eq:uuvsystemphys}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{NN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{SSS}(\overline{X}(t)),
\end{align}
\end{subequations}


Running one trial of system \eqref{eq:uuvsystemphys} on the real-time physics engine takes 3 minutes, as the system is running in real time. Thus, collecting 100 trials, which is a fairly small number in the statistical model checking world, takes 5 hours. This renders meaning statistical evaluations infeasible on this model. Instead, we view this model as the perturbed system in \eqref{eq:system_real} and we will instead derive a linearized model corresponding to \eqref{eq:system} next that we can use to collect data more efficiently. \footnote{In the end, however, we will collect data from both systems to support the claims made in Section \ref{sec:risk_gap} with respect to the risk verification gap between the systems in \eqref{eq:system} and \eqref{eq:system_real}.}

The linearization process is as follows. The UUV uses a pre-existing low level controller to drive the system to a specified heading, speed and depth. The desired heading, speed, depth commands are generated by a separate, high-level controller\footnote{These are the controllers we will synthesize and verify.}.  The goal of the linearization is to make the low level controllers and UUV physics appear linear to the high-level controller.  
Using data from the real-time physics engine, we identified a 4-th order linearized model of the UUV, which takes as input heading, speed, and depth commands (from the high-level controller) and outputs the actual heading, speed, and depth of the UUV. Note that by knowing the UUV's initial location and keeping track of the heading, speed, and depth over time one can compute the UUV's exact position and heading over time.
 

The equations in \eqref{eq:uuvsystemlin} show the dynamics of the linear simulator of the UUV. Here we have replaced the original dynamics $f$ with the linearized dynamics $f_{lin}$. The linearization also reduces the number of internal UUV states; so we have $\overline{X} = \begin{bmatrix} x_{uuv} & y_{uuv} & \theta_{uuv} &  v_{uuv} & d_{uuv} \end{bmatrix} ^{T}$, which contains the 2-D position, heading, speed and depth of the UUV, respectively. The $V$ term represents the linearization error of the system. Note that there is no measurement error term $W$, since the linearization does not affect the UUV sonar.
\begin{subequations}\label{eq:uuvsystemlin}
\begin{align}
    X(t+1)&=f_{lin}(C(t),\text{NN}(Y(t))), \; X(0)=X_0\\
    Y(t)&=\text{SSS}(X(t))
\end{align}
\end{subequations}



In order to get equations \eqref{eq:uuvsystemphys} and \eqref{eq:uuvsystemlin} to resemble equations \eqref{eq:system} and \eqref{eq:system_real}, we rewrite \eqref{eq:uuvsystemphys} as
\begin{subequations}\label{eq:uuvsystemphyserr}
\begin{align}
    \overline{X}(t+1)&=f_{lin}(\overline{X}(t),\text{NN}(\overline{Y}(t)))+V(\overline{X}(t),\cdot),  \; \overline{X}(0)=X_0,\\
    \overline{Y}(t)&=\text{SSS}(\overline{X}(t)),
\end{align}
\end{subequations}

So we have replaced the real-time physics engine as the linear simulator plus some linearization error term $V(\overline{X}(t),\cdot)$.


Next, we used the linearized system in \eqref{eq:uuvsystemlin} to train NN controllers to satisfy the objective in \eqref{eq:UUVspec} via RL. In particular, we  used the Twin Delayed Deep Deterministic Policy Gradients (TD3) algorithm \cite{Fujimoto2018} to train 4 NN controllers for guiding the UUV alongside a pipeline on the seafloor. The reward function for the RL used 4 additive terms. The first term gave a small penalty for each simulation step. The next gave a penalty for the magnitude of the commanded change in heading from the controller. The third gave a penalty for the difference between the UUV's distance to the pipeline and the desired distance to the pipeline. The final term adds a very large penalty if the UUV's distance to the pipe gets outside some safe interval. The size of the safe interval is what we altered for training the controllers. 
%using different reward functions in the RL \textcolor{red}{Give a short hint what exactly is different, and what the reward function is.}. 
Each NN consisted of 2 tanh layers, each of width 32.


\end{comment}




==> chapter/simulations.tex <==
\section{Case Studies}
\label{sec:simulations}

We continue our empirical validation of the F1/10 car, in addition to evaluating an unmanned underwater vehicle (UUV).



%We consider the following two systems for  empirical validations: an unmanned underwater vehicle (UUV) and an F-10th car.




\subsection{F1/10 Car}

The subsection continues the F1/10 case study introduced in Section~\ref{sec:F1TenthCaseStudy1}. In that portion of the case study, we used the statistical risk verification framework introduced in Section~\ref{risskk} to test 6 different NN controllers on a simulated model of the system. Now we analyze the same NN controllers on a more realistic LiDAR model and compare the results to the theory from Section~\ref{sec:risk_gap}.

%The second case study concerns an F1/10 car driving through a hallway with occasional turns. The car is equipped with a LiDAR system for sensing the distances to the hallway.  The STL requirement is specified with the following STL formula:
%\begin{align} \label{eq:F10spec_2}
%\phi_{F1/10} := G \left(d>d_{w} \right)
%\end{align}
%where $d$ is the distance of the car to the nearest wall and $d_w$ is the minimum allowed distance from the car to the wall.

%We trained 6 different NN controllers for navigating the car through the hallway, taking LiDAR rays as input and giving steering commands as output. We used a standard bicycle model as the model of the car for performing the RL. Our LiDAR model consisted of noisy range values and a fixed probability of a LiDAR randomly getting dropped before each trial.\footnote{A common issue with using LiDAR is that the rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We refer to this as a 'dropped' ray.} The specification for the car is that it never collides with the walls of the hallway, which is given in equation \eqref{eq:F10spec_2}. %We then ran 50000 trials of each controller navigating through a hallway with a right hand turn. 

%A common issue with using LiDAR data is that each LiDAR ray can be quite noisy. For example, the LiDAR rays can bounce off of reflective surfaces, causing the sensor to give very large distance readings. We accounted for this behavior in two ways. First, we altered our LiDAR model to randomly choose rays to drop for the duration of each run and ran 50000 trials for each controller. %From these data, we computed the VaR and CVaR risks for each of the controllers, which are shown in figure \ref{ex:f1-10VarMissingRays} and figure \ref{ex:f1-10CVarMissingRays}, respectively.

To simulate real-world LiDAR data, we  trained a GAN to approximate LiDAR readings from real-world LiDAR data. The GAN had a deconvoluational NN architecture \cite{radford2016} and was trained using the Wasserstein GAN algorithm \cite{arjovsky2017,gulrajani2017}. The GAN takes in the position and heading of the car and a 10 dimensional (random) seed and outputs an array of 21 LiDAR rays. 

Equation \eqref{eq:f1tenthsystemganlidar} shows the F1-10th with GAN LiDAR. The dynamics $f$ and state $\overline{X}$ are the same as in Section~\ref{sec:F1TenthCaseStudy1}. The GANLiDAR function is the GAN LiDAR model.
\begin{subequations}\label{eq:f1tenthsystemganlidar}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{DNN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{GANLiDAR}(\overline{X}(t)),
\end{align}
\end{subequations}

We now rewrite equation \eqref{eq:f1tenthsystemganlidar} to match the form of \eqref{eq:system_real}. The $W$ term accounts for the measurement differences between the simulated LiDAR and the GAN LiDAR. There is no $V$ term here, since the dynamics of the two system models are equivalent. 
\begin{subequations}\label{eq:f1tenthsystemganlidarerr}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{DNN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{SiMLiDAR}(\overline{X}(t)) + W(\overline{X}(t),\cdot),
\end{align}
\end{subequations}
where $W(\overline{X}(t),\cdot)=\text{GaNLiDAR}(\overline{X}(t)) - \text{SiMLiDAR}(X(t))$.






With this equation in hand, we ran 50000 trials of each of the 6 NN controllers operating in a hallway.  

%For ease of reference, we rewrite the simulated LiDAR model equation, originally given in \eqref{eq:f1tenthsystemsimlidar}. Recall that the $f$ dynamics function represents a kinematic bicycle model. The state is $X = \begin{bmatrix} x & y & v & \theta \end{bmatrix}^T$, where $x$ and $y$ are the car's position, $v$ is the car's velocity, and $\theta$ is the car's heading. The SiMLiDAR function is the simulated LiDAR model.
%\begin{subequations}\label{eq:f1tenthsystemsimlidar_2}
%\begin{align}
%    X(t+1)&=f(X(t),\text{DNN}(Y(t))), \; X(0)=X_0\\
%    Y(t)&=\text{SiMLiDAR}(X(t)),
%\end{align}
%\end{subequations}


From these data, we computed the VaR and CVaR risks for each of the controllers and LiDAR models using a single risk level of $\beta:=0.9$ and confidence of $1-\delta:=0.95$, which are shown in tables \ref{Tab:f1tenthVars} and \ref{Tab:f1tenthCVars}, along with the VaR and CVaR values from \eqref{eq:f1tenthsystemsimlidar} for ease of comparison.



\begin{table*}[h]
\caption{F1/10 VaR values for different LiDAR models under the specification given in \ref{eq:F10spec}.}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline Controller Name & Simulated LiDAR  & GAN Lidar & Color in Figures  \\ \hline
    1 & 0.1050 & 0.1306 & Black \\ \hline
    2 & 0.0776 & 0.0944 & Red \\ \hline
    3 & 0.1483 & 0.1435 & Green \\ \hline
    4 & 0.0165 & 0.1140 & Blue\\ \hline
    5 & 0.0368 & 0.0801 & Magenta\\ \hline
    6 & 0.0300 & 0.0727 & Cyan \\
    \hline
    \end{tabular}
    \label{Tab:f1tenthVars}
\end{table*}



\begin{table*}[h]
\caption{F1/10 CVaR values for different LiDAR models under the specification given in \ref{eq:F10spec}.}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline Controller Name & Simulated LiDAR  & GAN LiDAR & Color in Figures  \\ \hline
    1 & 0.1392 & 0.1986 & Black \\ \hline
    2 & 0.1108 & 0.1321 & Red \\ \hline
    3 & 0.1892 & 0.2038 & Green \\ \hline
    4 & 0.0805 & 0.1689 & Blue \\ \hline
    5 & 0.0746 & 0.1286 & Magenta \\ \hline
    6 & 0.0640 & 0.1249 & Cyan \\
    \hline
    \end{tabular}
    \label{Tab:f1tenthCVars}
\end{table*}


% simulation vars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_dont_hit_wall.png}
%\caption{Value-at-Risks (VaRs) for the STL robustness of 12 different RL-training f1tenth controllers.}
%\label{fig:f1-10Var}
%\end{figure}

% simulation cvars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_dont_hit_wall.png}
%\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness of 12 different RL-training f1tenth controllers.}
%\label{fig:f1-10CVar}
%\end{figure}

% missing lidar rays vars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_dont_hit_wall_missingRays.png}
%\caption{Value-at-Risks (VaRs) for the STL robustness of 12 different RL-training f1tenth controllers while randomly dropping lidar rays.}
%\label{fig:f1-10VarMissingRays}
%\end{figure}

% missing lidar rays cvars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_dont_hit_wall_missingRays.png}
%\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness of 12 different RL-training f1tenth controllers while randomly dropping lidar rays.}
%\label{fig:f1-10CVarMissingRays}
%\end{figure}


% gan vars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_dont_hit_wall_gan.png}
%\caption{Value-at-Risks (VaRs) for the STL robustness of 12 different RL-training f1tenth controllers, using a GAN to generate artificial LiDAR data.}
%\label{fig:f1-10VarGan}
%\end{figure}

% gan cvars
%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_dont_hit_wall_gan.png}
%\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness of 12 different RL-training f1tenth controllers, using a GAN to generate artificial LiDAR data.}
%\label{fig:f1-10CVarGan}
%\end{figure}



%In addition, we ran several real world traces (between 8 and 10) of the 12 controllers, for both modified and unmodified environments. The crash chances for each controller are shown in figures below.

%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/uncoveredCrashChances.png}
%\caption{Crash chances of the controllers for a clean environment.}
%\label{fig:f1-10Var}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/coveredCrashChances.png}
%\caption{Crash chances of the controllers for a modified environment.}
%\label{fig:f1-10CVar}
%\end{figure}

%All of the various var and cvars values are shown in the tables below.



We see that the controllers which perform well on the LiDAR model also perform well on the GAN LiDAR model, which is expected.





%With these two equations (\eqref{eq:f1tenthsystemsimlidar} and \eqref{eq:f1tenthsystemganlidarerr}) in hand, we generated 50000 traces for each of the 6 NNs we trained to guide the F1/10 car through a hallway with a right-hand turn.

%Second, we trained a GAN to approximate more realistic LiDAR readings using data of a real F1/10 car travelling around hallways. The GAN takes in the position and heading of the car and a 10 dimensional (random) seed and outputs an array of 21 LiDAR rays. Using this GAN, we then ran 50000 trials of each of the 12 NN controllers operating in a hallway. %From these data, we computed the VaR and CVaR risks for each of the controllers, which are shown in figure \ref{ex:f1-10VarGan} and figure \ref{ex:f1-10CVarGan}, respectively.  




%The GAN based lidar var values are consistent with the real world crash chances, which demonstrates how the risk robustness helps in addressing the sim2real gap.



Next, we varied the $\beta$ values for the VaR and CVaR metrics. These $\beta$ values control how much or little of the tail gets considered in the risk. Larger values only consider the extremes of the tails. The figures below show the different risk values for various controllers for both the simulated and GAN lidar models. Each controller gets its own color and the simulated LiDAR model values are shown as dots and the GAN LiDAR values are shown as stars. Note that we still observe that the controllers which perform better on the simulated LiDAR also perform well on the GAN LiDAR, although the correlation is not as clean as with the UUV case study. In particular, the blue controller shows very good CVaR values for smaller $\beta$ values, but as $\beta$ increases the performances becomes dominated by other controllers. The blue controller then performs much worse than those controllers on the GAN data. This illustrates the benefit of using risk measures analyzing systems in simulation. The very poor performance of the blue controller at the extreme tails of its robustness distribution properly indicated that it would not generalize well to the GAN LiDAR model.

\begin{figure}
\centering
\includegraphics[scale=0.5]{document/figures/vars_simReal_diffBetas.png}
\caption{Value at Risks (VaRs) for the F1/10 car under the specification given in \ref{eq:F10spec} for the simulated and GAN lidar models and various controllers.}
\label{fig:f1-10VarManyBetas}
\end{figure}


\begin{figure}
\centering
\includegraphics[scale=0.5]{document/figures/cvars_simReal_diffBetas.png}
\caption{Conditional Value at Risks (CVaRs) for the F1/10 car under the specification given in \ref{eq:F10spec} for the simulated and GAN lidar models and various controllers.}
\label{fig:f1-10CVarManyBetas}
\end{figure}



%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_simlidar_diffBetas.png}
%\caption{Value at Risks (VaRs) for the f1tenth car under specification 'do not hit the wall' for the simulated lidar model and various controllers.}
%\label{ex:f1-10SimLidarVarManyBetas}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_simlidar_diffBetas.png}
%\caption{Conditional Value at Risks (CVaRs) for the f1tenth car under specification 'do not hit the wall' for the simulated lidar model and various controllers.}
%\label{ex:f1-10SimLidarCVarManyBetas}
%\end{figure}



%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_missingrays_diffBetas.png}
%\caption{Value at Risks (VaRs) for the f1tenth car under specification 'do not hit the wall' for the 'missing rays' lidar model and various controllers.}
%\label{ex:f1-10MissingRaysVarManyBetas}
%\end{figure}



%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_missingrays_diffBetas.png}
%\caption{Conditional Value at Risks (CVaRs) for the f1tenth car under specification 'do not hit the wall' for the 'missing rays' lidar model and various controllers.}
%\label{ex:f1-10MissingRaysCVarManyBetas}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/vars_gan_diffBetas.png}
%\caption{Value at Risks (VaRs) for the f1tenth car under specification 'do not hit the wall' for the GAN lidar model and various controllers.}
%\label{ex:f1-10GANVarManyBetas}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[scale=0.5]{document/figures/cvars_gan_diffBetas.png}
%\caption{Conditional Value at Risks (VaRs) for the f1tenth car under specification 'do not hit the wall' for the GAN lidar model and various controllers.}
%\label{ex:f1-10GANCVarManyBetas}
%\end{figure}






\subsection{Unmanned Underwater Vehicle (UUV)}

%\textcolor{red}{General suggestion: I would suggest to use the terminology ``real-time physics engine'' for the gazebo simulator and ``linear simulator'' for the simulations based on the linear model throughout this section to align more with the terminology used before.}

\begin{figure}[ht!]
\centering
\includegraphics[scale=0.25]{document/figures/uuv/uuv_figure_topdown.png}
\caption{The UUV operating environment, both on paper and in the high fidelity physics engine. The pipelines are both shown in blue.}
\label{fig:uuv_fig}
\end{figure}


The UUV is tasked with following alongside a pipeline on the seafloor and using a side-scan sonar system to capture and inspect the pipeline, as shown in Figure \ref{fig:uuv_fig}. As the sonar works best in a certain range of distances from the pipeline, we consider the following requirement in STL that expresses expeditiousness:
%\begin{align} \label{eq:UUVspec}
%    \Phi_{UUV}:= &G (d<d_{u} \lor F_{[0,t_{UUV}]} d<d_{u}) \land \\
%    &G (d>d_{l} \lor F_{[0,t_{UUV}]} d>d_{l}) \nonumber
%\end{align}
\begin{align} \label{eq:UUVspec}
    \Phi_{UUV}:= &G \left[d<d_l \implies F_{[0,t_{UUV}]} \left(d \geq d_l \right) \right] \land \\
    &G \left[d>d_u \implies F_{[0,t_{UUV}]} \left(d \leq d_u \right) \right] \nonumber
\end{align}
%\textcolor{red}{1) Use STL terminology from background section, $F$ instead of $\square$, 2) use implication operator instead of disjunction re-formulation for better understanding - only few people are aware of the re-formulation.}
where $d$ is the UUV's distance to the pipeline in the plane, $d_u$ and $d_l$ are the upper and lower distances to the pipe which the UUV must lie within and $t_{UUV}$ is the amount of time in which the UUV is allowed to leave this distance range.\footnote{For example, the UUV may need to avoid obstacles, in which case it is allowed to lose the pipe for a small period of time.}



We consider a high-fidelity UUV model based on the ROS-Gazebo real-time physics engine presented in \cite{Manhaes2016}. As gathering data on real-time systems is time-consuming, we view this model as the perturbed system in \eqref{eq:system_real} and we will instead derive a linearized model corresponding to \eqref{eq:system} next that we can use to collect data more efficiently. In the end, however, we will collect data from both systems to support the claims made in Section \ref{sec:risk_gap} with respect to the risk gap between the systems in \eqref{eq:system} and \eqref{eq:system_real}.

The linearization process is as follows. The UUV uses a pre-existing low level controller to drive the system to a specified heading, speed and depth. The desired heading, speed, depth commands are generated by a separate, high-level controller\footnote{These are the controllers we will synthesize and verify.}.  The goal of the linearization is to make the low level controllers and UUV physics appear linear to the high-level controller.  
Using data from the real-time physics engine, we identified a 4-th order linearized model of the UUV, which takes as input heading, speed, and depth commands (from the high-level controller) and outputs the actual heading, speed, and depth of the UUV. Note that by knowing the UUV's initial location and keeping track of the heading, speed, and depth over time one can compute the UUV's exact position and heading over time.
 


%The linearization process is as follows. The UUV in question uses PID controllers to drive the system to a specified heading, speed and depth. \textcolor{red}{1) I guess heading, speed and depth are the states $X$? Is there no $x$ and $y$ coordinates? Otherwise I don't see how $d$ above is defined. 2) Do I understand it correctly that the PID is only used for obtaining the linearized model? It may be confusing to have two controller, i.e., PID and NN. 3) What are the outputs of the function $u$, i.e, the inputs of the system?}. Using data from this simulator, we identified a 4-th order linearized model \textcolor{red}{We need to emphasize that this corresponds to (3).}  of the UUV \textcolor{red}{linearized around what?}, which takes as input heading, speed, and depth commands and outputs the actual heading, speed, and depth of the UUV \textcolor{red}{I think I'm not entirely following}. 
 
The equations in \eqref{eq:uuvsystemphys} show the real-time physics engine UUV dynamics. In this case, $Y(t) = \begin{bmatrix} d \\ \theta \end{bmatrix}$ is the distance and heading of the UUV with respect to the pipeline being tracked. The dynamics $f$ and state $X(t)$ are internal to the real-time physics engine, so we keep them general due to space constraints. The SSS function stands for side scan sonar, which is what the UUV uses to detect and track the pipeline. Finally, the DNN function is our DNN controller for the UUV.
\begin{subequations}\label{eq:uuvsystemphys}
\begin{align}
    \overline{X}(t+1)&=f(\overline{X}(t),\text{DNN}(\overline{Y}(t))), \; \overline{X}(0)=X_0\\
    \overline{Y}(t)&=\text{SSS}(\overline{X}(t)),
\end{align}
\end{subequations}


The equations in \eqref{eq:uuvsystemlin} show the dynamics of the linear simulator of the UUV. Here we have replaced the original dynamics $f$ with the linearized dynamics $f_{lin}$. The linearization also reduces the number of internal UUV states; so we have $\overline{X} = \begin{bmatrix} x_{uuv} & y_{uuv} & \theta_{uuv} &  v_{uuv} & d_{uuv} \end{bmatrix} ^{T}$, which contains the 2-D position, heading, speed and depth of the UUV, respectively. The $V$ term represents the linearization error of the system. Note that there is no measurement error term $W$, since the linearization does not affect the UUV sonar.
 \begin{subequations}\label{eq:uuvsystemlin}
\begin{align}
    X(t+1)&=f_{lin}(C(t),\text{DNN}(Y(t))), \; X(0)=X_0\\
    Y(t)&=\text{SSS}(X(t))
\end{align}
\end{subequations}


In order to get equations \eqref{eq:uuvsystemphys} and \eqref{eq:uuvsystemlin} to resemble equations \eqref{eq:system} and \eqref{eq:system_real}, we rewrite \eqref{eq:uuvsystemphys} as
\begin{subequations}\label{eq:uuvsystemphyserr}
\begin{align}
    \overline{X}(t+1)&=f_{lin}(\overline{X}(t),\text{DNN}(\overline{Y}(t)))+V(\overline{X}(t),\cdot),  \; \overline{X}(0)=X_0,\\
    \overline{Y}(t)&=\text{SSS}(\overline{X}(t)),
\end{align}
\end{subequations}

So we have replaced the real-time physics engine as the linear simulator plus some linearization error term $V(\overline{X}(t),\cdot)$.

Having systems \eqref{eq:uuvsystemlin} and \eqref{eq:uuvsystemphyserr} at hand, our ultimate goal is to verify DNN controllers that have been trained for these systems and with the objective in \eqref{eq:UUVspec}. In particular, we  used the Twin Delayed Deep Deterministic Policy Gradients (TD3) algorithm \cite{Fujimoto2018} to train 4 NN controllers for guiding the UUV alongside a pipeline on the seafloor. The reward function for the RL used 4 additive terms. The first term gave a small penalty for each simulation step. The next gave a penalty for the magnitude of the commanded change in heading from the controller. The third gave a penalty for the difference between the UUV's distance to the pipeline and the desired distance to the pipeline. The final term adds a very large penalty if the UUV's distance to the pipe gets outside some safe interval. The size of the safe interval is what we altered for training the controllers. 
%using different reward functions in the RL \textcolor{red}{Give a short hint what exactly is different, and what the reward function is.}. 
Each NN consisted of 2 tanh layers, each of width 32.

To now verify these DNN controllers, each of them was used to generate 5000 runs of the linear simulator and 300 runs of the real-time physics engine, each corresponding to 3 minutes of data per run.  Finally, the STL robustness risk of the STL specification in \eqref{eq:UUVspec}  is estimated as explained in Section ~\ref{sec:stoch} for the VaR and the CVaR and for a risk level of $\beta:=0.9$ and  a confidence of $1-\delta:=0.95$. The results are shown in table \ref{Tab:UUVRisks}. The controllers which exhibit higher risk on the linear simulator also exhibit higher risk on the real-time physics engine for both VaR and CVaR, supporting the claims from Section \ref{sec:risk_gap}. 
%\textcolor{red}{I believe that we here have to quantifiy a little more the differences between these systems. As I don't fully understand the linearization yet, this is sth we should discuss.} 
This offers empirical evidence that systems which exhibit lower robustness risk in simulation will also exhibit lower robustness risk in the real world.


%UUV case study overview:




%We have a high fidelity model of a UUV in ROS-Gazebo. In the simulator, a UUV operates via heading-speed-depth commands. A bunch of simulation data was collected and a 4th order linearized model of the UUV was obtained via SysID. This model maps HSD commands to the heading-speed-depth of the UUV. Then, reinforcement learning was used to learn a controller for the UUV to follow a pipeline along some offset. This controller was then verified on the linearized model using Verisig.

%We want to use data collected from the linearized model to compute risk bounds for the system for a range of NN based controllers. Then we want to run these controllers on the actual simulator to see how they perform in a more realistic environment. In particular, we aim to show that controllers which are more robust on the linearized model are also more robust on the actual model. 

%The table below shows the var and cvar results for our experiments for different safety range parameters used to train the NN controllers.

\begin{table*}[h]
\caption{UUV risks for a real-time physics engine and a linear simulator for specification \ref{eq:UUVspec}.}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline \specialcell{Safety \\ Range} & \specialcell{Linear \\ Simulator VaR} & \specialcell{Real-Time Physics \\ Engine VaR} & \specialcell{Linear \\ Simulator CVaR} & \specialcell{Real-Time Physics \\ Engine CVaR} \\ \hline
    10 & -10.1215 & -7.9380 & -7.0261 & -4.3691 \\ \hline
    15 & -1.8944 & 5.0788 & 2.3087 & 13.1208 \\ \hline
    30 & -8.2857 & -6.0316 & -5.2708 & 8.7808 \\ \hline
    50 & -10.0697 & -8.3995 & -7.3678 & -5.4930 \\
    \hline
    \end{tabular}
    \label{Tab:UUVRisks}
\end{table*}



%\begin{table*}[h]
%\caption{UUV risks for a high-fidelity simulator and a linearized model for the always safe specification.}
%    \centering
%    \begin{tabular}{|c|c|c|c|c|}
%    \hline Safety Range & Linear Model VaR & Simulation VaR & Linear Model CVaR & Simulation CVaR  \\ \hline
%    10 & -10.081558712502733 & -7.894395070282689 & -7.018185402480389 & -4.369071314298114 \\ \hline
%    15 & -1.894381976464869 & 5.078759635452745 & 2.3086623530430073 & 13.120824002217459 \\ \hline
%    30 & -8.285720602680037 & -5.8562478139734235 & -5.270781390235433 & 81.65188007331035 \\ \hline
%    50 & -10.028407645407007 & -8.36976298396543 & -7.362237771578118 & -5.342417627238612 \\
%    \hline
%    \end{tabular}
%    \label{Tab:UUVRisks_always}
%\end{table*}


Next, we varied the risk level $\beta$  for the VaR and CVaR metrics. These $\beta$ values control how much or little of the tail gets considered in the risk. Larger values only consider the extremes of the tails. Figures \ref{fig:uuvVaRsManyBetas} and \ref{fig:uuvCVaRsManyBetas} show the VaR and CVaR values, respectively, for both the linear simulator and real-time physics engine and different controllers for the specification given in \ref{eq:UUVspec}. In both figures, each controller gets its own color, and risks on the linear simulator are dots, while risks on the real-time physics engine are stars. These figures both show that controllers which exhibit low risk values on the linear simulator also exhibit low risk values on the real-time physics engine and vice versa, and are hence in line with the results in Section \ref{sec:risk_gap}.


% linear model vars
\begin{figure}
\centering
\includegraphics[scale=0.5]{document/figures/vars_over_50_implies_under_50_10_seconds_and_under_10_implies_over_10_10_seconds_diffBetas.png}
\caption{Value-at-Risks (VaRs) for the STL robustness under the specification in \ref{eq:UUVspec} of the 4 different controllers on both UUV models for varied $\beta$ parameters.}
\label{fig:uuvVaRsManyBetas}
\end{figure}


% linear model cvars
\begin{figure}
\centering
\includegraphics[scale=0.5]{document/figures/cvars_over_50_implies_under_50_10_seconds_and_under_10_implies_over_10_10_seconds_diffBetas.png}
\caption{Conditional Value-at-Risks (CVaRs) for the STL robustness under the specification in \ref{eq:UUVspec} of the 4 different controllers on both UUV models for varied $\beta$ parameters.}
\label{fig:uuvCVaRsManyBetas}
\end{figure}





